Unsupervised Reinforcement Learning in Multiple Environments

Several recent works have been dedicated to unsupervised reinforcement learning in a single environment, in which a policy is first pre-trained with unsupervised interactions, and then fine-tuned towards the optimal policy for several downstream supervised tasks defined over the same environment. Along this line, we address the problem of unsupervised reinforcement learning in a class of multiple environments, in which the policy is pre-trained with interactions from the whole class, and then fine-tuned for several tasks in any environment of the class. Notably, the problem is inherently multi-objective as we can trade off the pre-training objective between environments in many ways. In this work, we foster an exploration strategy that is sensitive to the most adverse cases within the class. Hence, we cast the exploration problem as the maximization of the mean of a critical percentile of the state visitation entropy induced by the exploration strategy over the class of environments. Then, we present a policy gradient algorithm, $\alpha$MEPOL, to optimize the introduced objective through mediated interactions with the class. Finally, we empirically demonstrate the ability of the algorithm in learning to explore challenging classes of continuous environments and we show that reinforcement learning greatly benefits from the pre-trained exploration strategy w.r.t. learning from scratch.

==> contents/figures/old/gridslope_alpha_sensitivity.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{contents/plot_files/img/gridslope_percentile_dist.pdf}
    \caption{Percentile distribution}
    \label{fig:gridslope_perc_dist}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.6\textwidth}
    \centering
    \includegraphics[width=\textwidth]{contents/plot_files/img/gridslope_percentiles_comparison.pdf}
    \caption{$\alpha$ comparison}
    \label{fig:gridslope_percentiles_comparison}
    \end{subfigure}
    \caption{$\textbf{(a)}$ Percentage of mini-batches inside the $\alpha$-percentile ($\alpha = 0.35$) for each configuration throughout the training. The two dotted lines represent the quantity that one could expect if considering the distribution $p_{\vcmp} = [0.8, 0.2]$. $\textbf{(b)}$ Comparison between optimal policies trained with different value of $\alpha$. (95\% c.i. over 4 runs, $N_{traj} = 200$, $T = 400$).}
    \label{fig:alpha_sensitivity}
\end{figure*}

==> contents/figures/old/gridslope_configs.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[scale=0.7]
    \draw (0,0) -- (4,0) -- (4,4) -- (0,4) -- cycle;
    \fill[yellow] (0.3,3.7) -- (0.8,3.7) -- (0.8,3.2) -- (0.3,3.2) -- cycle;
    % bottom-left
    \draw[line] (0.3,0.3) -- (0.3,1.75);
    \draw[line] (0.3,1.75) -- (1.05,1.75);
    \draw[line] (1.35,1.75) -- (1.75,1.75);
    \draw[line] (1.75,1.75) -- (1.75,1.35);
    \draw[line] (1.75,1.05) -- (1.75,0.3);
    \draw[line] (1.75,0.3) -- (0.3,0.3);
    
    % top-left
    \draw[line] (0.3,2.25) -- (0.3,3.7);
    \draw[line] (0.3,3.7) -- (1.75,3.7);
    \draw[line] (1.75,3.7) -- (1.75,2.95);
    \draw[line] (1.75,2.25) -- (1.75,2.65);
    \draw[line] (1.75,2.25) -- (1.35,2.25);
    \draw[line] (1.05,2.25) -- (0.3,2.25);
    
    % top-right
    \draw[line] (2.25,2.25) -- (2.25,2.65);
    \draw[line] (2.25,2.95) -- (2.25,3.7);
    \draw[line] (2.25,3.7) -- (3.7,3.7);
    \draw[line] (3.7,3.7) -- (3.7,2.25);
    \draw[line] (3.7,2.25) -- (2.95,2.25);
    \draw[line] (2.65,2.25) -- (2.25,2.25);
    
    % bottom-right
    \draw[line] (2.25,0.3) -- (2.25, 1.05);
    \draw[line] (2.25,1.35) -- (2.25, 1.75);
    \draw[line] (2.25,1.75) -- (2.65,1.75);
    \draw[line] (2.95,1.75) -- (3.7,1.75);
    \draw[line] (3.7,1.75) -- (3.7,0.3);
    \draw[line] (3.7,0.3) -- (2.25,0.3);
    
    % Hallways
    \draw[line] (1.05,1.75) -- (1.05,2.25);
    \draw[line] (1.35,1.75) -- (1.35,2.25);
    
    \draw[line] (1.75,2.95) -- (2.25,2.95);
    \draw[line] (1.75,2.65) -- (2.25,2.65);
    
    \draw[line] (2.65,1.75) -- (2.65,2.25);
    \draw[line] (2.95,1.75) -- (2.95,2.25);
    
    \draw[line] (1.75,1.35) -- (2.25,1.35);
    \draw[line] (1.75,1.05) -- (2.25,1.05);
    
    % Slope
    \draw[dashed] (0,2) -- (4,2);
    
    \node[text=blue] at(0.5,3.4) {$\downarrow$};
    \node[text=blue] at(1.0,3.4) {$\downarrow$};
    \node[text=blue] at(1.5,3.4) {$\downarrow$};
    \node[text=blue] at(0.5,2.7) {$\downarrow$};
    \node[text=blue] at(1.0,2.7) {$\downarrow$};
    \node[text=blue] at(1.5,2.7) {$\downarrow$};
    
    \node[text=blue] at(2.45,3.4) {$\downarrow$};
    \node[text=blue] at(2.95,3.4) {$\downarrow$};
    \node[text=blue] at(3.45,3.4) {$\downarrow$};
    \node[text=blue] at(2.45,2.7) {$\downarrow$};
    \node[text=blue] at(2.95,2.7) {$\downarrow$};
    \node[text=blue] at(3.45,2.7) {$\downarrow$};
    
    \node[text=blue] at(1.975,2.8) {$\downarrow$};
    
    \node[text=blue] at(1.2,2.2) {$\downarrow$};
    \node[text=blue] at(2.8,2.2) {$\downarrow$};
\end{tikzpicture}
\qquad
\begin{tikzpicture}[scale=0.7]
    \draw (0,0) -- (4,0) -- (4,4) -- (0,4) -- cycle;
    \fill[yellow] (0.3,3.7) -- (0.8,3.7) -- (0.8,3.2) -- (0.3,3.2) -- cycle;
    % bottom-left
    \draw[line] (0.3,0.3) -- (0.3,1.75);
    \draw[line] (0.3,1.75) -- (1.05,1.75);
    \draw[line] (1.35,1.75) -- (1.75,1.75);
    \draw[line] (1.75,1.75) -- (1.75,1.35);
    \draw[line] (1.75,1.05) -- (1.75,0.3);
    \draw[line] (1.75,0.3) -- (0.3,0.3);
    
    % top-left
    \draw[line] (0.3,2.25) -- (0.3,3.7);
    \draw[line] (0.3,3.7) -- (1.75,3.7);
    \draw[line] (1.75,3.7) -- (1.75,2.95);
    \draw[line] (1.75,2.25) -- (1.75,2.65);
    \draw[line] (1.75,2.25) -- (1.35,2.25);
    \draw[line] (1.05,2.25) -- (0.3,2.25);
    
    % top-right
    \draw[line] (2.25,2.25) -- (2.25,2.65);
    \draw[line] (2.25,2.95) -- (2.25,3.7);
    \draw[line] (2.25,3.7) -- (3.7,3.7);
    \draw[line] (3.7,3.7) -- (3.7,2.25);
    \draw[line] (3.7,2.25) -- (2.95,2.25);
    \draw[line] (2.65,2.25) -- (2.25,2.25);
    
    % bottom-right
    \draw[line] (2.25,0.3) -- (2.25, 1.05);
    \draw[line] (2.25,1.35) -- (2.25, 1.75);
    \draw[line] (2.25,1.75) -- (2.65,1.75);
    \draw[line] (2.95,1.75) -- (3.7,1.75);
    \draw[line] (3.7,1.75) -- (3.7,0.3);
    \draw[line] (3.7,0.3) -- (2.25,0.3);
    
    % Hallways
    \draw[line] (1.05,1.75) -- (1.05,2.25);
    \draw[line] (1.35,1.75) -- (1.35,2.25);
    
    \draw[line] (1.75,2.95) -- (2.25,2.95);
    \draw[line] (1.75,2.65) -- (2.25,2.65);
    
    \draw[line] (2.65,1.75) -- (2.65,2.25);
    \draw[line] (2.95,1.75) -- (2.95,2.25);
    
    \draw[line] (1.75,1.35) -- (2.25,1.35);
    \draw[line] (1.75,1.05) -- (2.25,1.05);
    
    % Slope
    \draw[dashed] (0,2) -- (4,2);
    
    \node[text=red] at(0.5,3.4) {$\uparrow$};
    \node[text=red] at(1.0,3.4) {$\uparrow$};
    \node[text=red] at(1.5,3.4) {$\uparrow$};
    \node[text=red] at(0.5,2.7) {$\uparrow$};
    \node[text=red] at(1.0,2.7) {$\uparrow$};
    \node[text=red] at(1.5,2.7) {$\uparrow$};
    
    \node[text=red] at(2.45,3.4) {$\uparrow$};
    \node[text=red] at(2.95,3.4) {$\uparrow$};
    \node[text=red] at(3.45,3.4) {$\uparrow$};
    \node[text=red] at(2.45,2.7) {$\uparrow$};
    \node[text=red] at(2.95,2.7) {$\uparrow$};
    \node[text=red] at(3.45,2.7) {$\uparrow$};
    
    \node[text=red] at(1.975,2.8) {$\uparrow$};
    
    \node[text=red] at(1.2,2.2) {$\uparrow$};
    \node[text=red] at(2.8,2.2) {$\uparrow$};
\end{tikzpicture}
\caption{Illustration of the GWS (left) and the GWN (right) configurations of the \emph{GridWorld with Slope} setting. The arrows represent the slope, yellow boxes indicate the initial state distribution.}
\label{fig:gridslope_configs}
\end{figure}

==> contents/figures/old/gridslope_entropy_comparison.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \includegraphics[scale=1]{contents/plot_files/img/gridslope_hist_ent_multi.pdf}
        \caption{Multiple}
        \label{fig:gridslope_hist_ent_multi}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \includegraphics[scale=1]{contents/plot_files/img/gridslope_hist_ent_north.pdf}
        \caption{GWN}
        \label{fig:gridslope_hist_ent_north}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \includegraphics[scale=1]{contents/plot_files/img/gridslope_hist_ent_south.pdf}
        \caption{GWS}
        \label{fig:gridslope_hist_ent_south}
    \end{subfigure}
    \caption{Comparison between the optimal policies of each tested configuration: we plot the $\mathcal{E}_{\vcmp}^1(\pi)$ ($\alpha = 1$) obtained by running each optimal policy on GridWorld with both the environments sampled according to $p_{\vcmp} = [0.8,0.2]$ in \textbf{(a)}, on the \emph{adversarial} $GWN$ in \textbf{(b)} and on the \emph{easier} $GWS$ in \textbf{(c)}. The dashed line in \textbf{(b)} and \textbf{(c)} represents the optimal value of $\mathcal{E}_{\vcmp}^1(\pi)$ in that specific configuration. (95\% c.i. over 4 runs, $N_{traj} = 200$, $T = 400$).}
    \label{fig:gridslope_entropy_comparison}
\end{figure*}

==> contents/figures/old/gridslope_entropy_dist_and_baseline.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{contents/plot_files/img/gridslope_ent_dist.pdf}
        \caption{$\mathcal{E}_{\vcmp}$}
        \label{fig:gridslope_entropy_distribution}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{contents/plot_files/img/gridslope_baseline.pdf}
        \caption{Baseline}
        \label{fig:gridslope_baselines_comparison}
    \end{subfigure}
    \caption{In \textbf{(a)} we show how the metric $\mathcal{E}_{\vcmp}$ is distributed, highlighting the loss of the \emph{double-tail} in MEMENTO ($p_{\vcmp} = [0.8, 0.2])$. In \textbf{(b)} we provide a comparison supporting the choice of our baseline $b = - \var (H_\tau)$. (95\% c.i. over 4 runs, $N_{traj} = 200$, $T = 400$).}
    \label{fig:gridslope_entropy_dist_and_baseline}
\end{figure*}

==> contents/figures/old/gridslope_perc_dist.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.55\columnwidth]{contents/plot_files/img/gridslope_percentile_dist.pdf}
    \caption{Distribution of mini-batches inside the $\alpha$-percentile ($\alpha = 0.35$). We plot the number of batches that fall into the the $\alpha$-percentile for each configuration throughout the training. The two dotted lines represent the quantity that one could expect if considering the distribution $p_{\vcmp} = [0.8, 0.2]$ (95\% c.i. over 4 runs, $N_{traj} = 200$, $T = 400$).}
    \label{fig:gridslope_perc_dist}
\end{figure}

==> contents/figures/old/gridslope_percentiles_comparison.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.9\columnwidth]{contents/plot_files/img/gridslope_percentiles_comparison.pdf}
    \caption{Comparison between optimal policies trained with different value of $\alpha$ (95\% c.i. over 4 runs, $N_{traj} = 200$, $T = 400$).}
    \label{fig:gridslope_percentiles_comparison}
\end{figure}

==> contents/figures/old/multigrid_entropy_comparison.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{contents/plot_files/img/multigrid_entropy_estimation.pdf}
        \caption{Adversarial}
        \label{fig:multigrid_entropy_comparison_adv}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{contents/plot_files/img/multigrid_entropy_estimation_all_configs.pdf}
        \caption{Multiple}
        \label{fig:multigrid_entropy_comparison_multi}
    \end{subfigure}
    \caption{Comparison between MEMENTO and risk-neutral: we plot both $\mathcal{E}_{\vcmp}$ and $\mathcal{E}_{\vcmp}^{\alpha}$ with $\alpha = 0.1$ obtained by running the optimal policies on $\textbf{(a)}$ the \emph{adversarial} configuration and $\textbf{(b)}$ with all the 10 configurations, each one sampled with probability $p_{\cmp} = 0.1$. (95\% c.i. over 4 runs, $N_{traj} = 500$, $T = 400$).}
    \label{fig:multigrid_entropy_comparison}
\end{figure*}

==> contents/figures/old/multigrid_goal_rl.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.85]{contents/plot_files/img/multigrid_goal_rl.pdf}
    \caption{Comparison of the average return as a function of learning epochs achieved by TRPO with MEMENTO initialization, TRPO with a risk-neutral policy as initialization and TRPO from scratch over a set of sparse-reward RL tasks in the adversarial configuration (95\% c.i. over 54 sampled goal locations).}
    \label{fig:multigrid_goal_rl}
\end{figure}

==> contents/figures/related_work.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{contents/images/related_work.png}
    \caption{Where our work (star) stands in the literature.}
    \label{fig:related_work}
\end{figure}

==> contents/sections/conclusions.tex <==
% In this paper, we addressed the problem of learning to explore a class of multiple reward-free environments with a unique general strategy. First, we cast the problem into the familiar MSVE framework, where we considered the maximization of a critical percentile of the state visitation entropy. Then, we presented MEMENTO, a policy gradient algorithm to optimize the exploration objective via mediated interactions with the class of environments. Finally, we provided an extensive experimental analysis to show the ability of MEMENTO in learning to explore challenging classes of continuous environments and to highlight the benefit that the resulting exploration strategy brings to RL problems specified over the same classes.
In this paper, we addressed the problem of learning to explore a class of multiple reward-free environments with a unique general strategy. First, we formulated the problem within a tractable MSVE objective with percentile sensitivity. Then, we presented a policy gradient algorithm to optimize this objective. Finally, we provided an extensive experimental analysis to show its ability in learning to explore and the benefits it brings to subsequent RL problems.
We believe that this paper motivates the importance of designing specific solutions to the relevant reward-free exploration problem over multiple environments.

%As a final note, it is worth mentioning an alternative problem formulation in which MEMENTO can be employed with benefit. 
%Especially, we could replace the class of environments of our setting with a single CMP specified under uncertainty~\citep{satia1973markovian}, and deal with the \emph{robust reward-free exploration} problem with little or no modifications to MEMENTO.
% On an orthogonal line, one could pursue reward-free exploration of a class of multiple \emph{vision-based domains}. In this case, MEMENTO could be employed in combination with a proper metric learned over images, as proposed in~\citep{anonymous2021unsupervised} for an environment-specific setting.


==> contents/sections/experiments.tex <==
In this section, we provide an extensive empirical evaluation of the proposed methodology over the two-phase learning process described in Figure~\ref{fig:problem}, which is organized as follows:
\begin{itemize} \compresslist
    \item[\ref{sec:experiments_learning_to_explore_illlustrative}]
    We show the ability of our method in learning to explore a class of illustrative continuous gridworlds, emphasizing the importance of the percentile sensitivity;
    \item[\ref{sec:experiments_alpha_sensitivity}]
    We discuss how the choice of the percentile of interest affects the exploration strategy;
    \item[\ref{sec:experiments_rl_illustrative}]
    We highlight the benefit that the exploration strategy provides to RL on the same class;
    \item[\ref{sec:experiments_scalability_class}]
    We verify the ability of our method to scale with the size of the class of environments, by considering a class of 10 continuous gridworlds;
    \item[\ref{sec:experiments_scalability_dimension}]
    We verify the ability of our method to scale with the dimensionality of the environments in the class, by considering a class of 29D continuous control Ant domains;
    \item[\ref{sec:experiments_scalability_vision}] We verify the ability of our method to scale with visual inputs, by considering a class of 147D MiniGrid~\citep{chevalier2018minimalistic} domains;
    \item[\ref{sec:experiments_meta}]
    We show that the exploration strategy learned with our approach is superior for RL \wrt a policy meta-trained with MAML~\citep{finn2017model, gupta2018unsupervised} on the same class.
\end{itemize}
A thorough description of the experimental setting is provided in Appendix~\ref{apx:experiments}.

\input{contents/figures/gridslope}
\subsection{Learning to Explore Multiple Environments with Percentile Sensitivity}
\label{sec:experiments_learning_to_explore_illlustrative}
In this section, we consider a class $\vcmp$ composed of two different configurations of a continuous gridworld domain with 2D states and 2D actions, which we call the \emph{GridWorld with Slope}. In each configuration, the agent navigates through four rooms connected by narrow hallways, by choosing a (bounded) increment along the coordinate directions. A visual representation of the setting can be found in Figure~\ref{fig:gridslope_illustration}, where the shaded areas denote the initial state distribution and the arrows render a slope that favors or contrasts the agent's movement. The configuration on the left has a south-facing slope, and thus it is called GridWorld with South slope (GWS). Instead, the one on the right is called GridWorld with North slope (GWN) as it has a north-facing slope. This class of environments is unbalanced (and thus interesting to our purpose) for two reasons: First, the GWN configuration is more challenging from a pure exploration standpoint, since the slope prevents the agent from easily reaching the two bottom rooms; secondly, the distribution over the class is also unbalanced, as it is $p_{\vcmp} = [Pr(\text{GWS}), Pr(\text{GWN})] = [0.8, 0.2]$.
In this setting, we compare  MEMENTO against \emph{Neutral}, which is a simplified version of MEMENTO with $\alpha = 1$,\footnote{The pseudocode is identical to Algorithm~\ref{alg:memento} except that all trajectories affect the gradient estimate in~\eqref{eq:policy_gradient_estimator}.} to highlight the importance of percentile sensitivity \wrt a na\"ive approach to the multiple environments scenario. The methods are evaluated in terms of the state visitation entropy $\mathcal{E}_{\vcmp}^1$ induced by the exploration strategies they learn.

In Figure~\ref{fig:gridslope_exploration}, we compare the performance of the optimal exploration strategy obtained by running MEMENTO ($\alpha=0.2$) and Neutral ($\alpha=1$) for 150 epochs on the GridWorld with Slope class ($p_{\vcmp} = [0.8, 0.2]$). We show that the two methods achieve a very similar expected performance over the class (Figure~\ref{fig:gridslope_exploration_all}). However, this expected performance is the result of a (weighted) average of very different contributions. As anticipated, Neutral has a strong performance in GWS ($p_{\vcmp} = [1, 0]$, Figure~\ref{fig:gridslope_exploration_south}), which is close to the configuration-specific optimum (dashed line), but it displays a bad showing in the adverse GWN ($p_{\vcmp} = [0, 1]$, Figure~\ref{fig:gridslope_exploration_north}). Conversely, MEMENTO learns a strategy that is much more robust to the configuration, showing a similar performance in GWS and GWN, as the percentile sensitivity prioritizes the worst case during training. 
To confirm this conclusion, we look at the actual distribution that is generating the expected performance in Figure~\ref{fig:gridslope_exploration_all}. In Figure~\ref{fig:gridslope_empirical_distribution}, we provide the empirical distribution of the trajectory-wise performance ($H_\tau$), considering a batch of 200 trajectories with $p_{\vcmp} = [0.8, 0.2]$. It clearly shows that Neutral is heavy-tailed towards lower outcomes, whereas MEMENTO concentrates around the mean. \emph{This suggests that with a conservative choice of $\alpha$ we can induce a good exploration outcome for every trajectory (and any configuration), while without percentile sensitivity we cannot hedge against the risk of particularly bad outcomes.} However, let us point out that not all classes of environments would expose such an issue for a na\"ive, risk-neutral approach (see Appendix~\ref{apx:counterexample} for a counterexample), but it is fair to assume that this would arguably generalize to any setting where there is an imbalance (either in the hardness of the configurations, or in their sampling probability) in the class. These are the settings we care about, as they require nuanced solutions (\eg MEMENTO) for scenarios with multiple environments.
\input{contents/figures/gridslope_rl}

% we provide a comparison directed at showing empirically the claim presented in Section 4. We show that the CVaR optimization as in (\ref{eq:exp_risk_averse}), combined to the sampling procedure in $\vcmp$, leads to a more robust exploratory policy, i.e. able to generalize through different environments, without suffering a drop in performance due to some adversarial configurations.
% We carry out the evaluation on a custom version of GridWorld (2D states, 2D actions), which we coded from scratch. An illustration to facilitate the comprehension of the setting is shown in Figure \ref{fig:gridslope_illustration}. The agent can move inside a map composed of four rooms connected by four hallways, by choosing at each step how much to move on the x and y axes. There are two configurations sharing this spatial context, each one characterized by a different level of complexity: we denote the \emph{easy} one as $GWS$ (GridWorld with South slope), since it is characterized by a south-facing slope, while $GWN$ (GridWorld with North slope) is the \emph{adversarial} one and it is characterized by a north-facing slope. Both the slopes are applied only in the upper half of the environment. Because of the way in which the initial position of the agent is determined, $GWN$ has a higher level of complexity, since at least in the first epochs the agent will continuously collide with the top-border of the environment, leading in general to a much more lower entropy \wrt to $GWS$. The two environments $GWS$ and $GWN$ are drawn according to a specified non-uniform distribution $p_{\vcmp} = [0.8, 0.2]$, meaning that the \emph{adversarial} configuration is sampled only with a probability of $0.2$, as a representative of the \emph{worst-case} scenario.
% In Figure \ref{fig:gridslope_exploration} we depict a comparison showing the performance of the optimal policy in each configuration. From Figure \ref{fig:gridslope_exploration_all} one can see that MEMENTO is able to obtain an exploration comparable to the one of the risk-neutral approach in the \emph{multi-environment} scenario. Figure \ref{fig:gridslope_exploration_north} considers the \emph{adversarial} configuration $GWN$ ($p_{\vcmp} = [0, 1]$) and it demonstrates that our approach outclasses the risk-neutral one, which instead obtains a performance comparable to the policy trained with only south-facing slope. Finally, Figure \ref{fig:gridslope_exploration_south} illustrates how our approach, although performing worse than the risk-neutral one, still results in a good exploration also in $GWS$ ($p_{\vcmp} = [1, 0]$): crucially, the gap here is definitely smaller than the gap in Figure \ref{fig:gridslope_exploration_north}. Overall, it is clear that MEMENTO manages to learn a policy which is is able to crosswise explore $\vcmp$, without suffering the presence of a challenging configuration. In order to corroborate such result, in Figure \ref{fig:gridslope_empirical_distribution} we give a visualization of the way in which the metric $\mathcal{E}_{\vcmp}$ is distributed, plotting the number of mini-batches that fall in a specific range of values. Crucially, the \emph{double-tail} behaviour of the risk-neutral policy disappears with MEMENTO, meaning the \emph{elimination of the risk} in exchange for a small lowering of the average performance. In Figure \ref{fig:gridslope_alpha_composition} we instead show the proportion according to which the mini-batches fall in the $\alpha$-percentile. Clearly, the percentage of mini-batches containing trajectories sampled from the \emph{adversarial} configuration $GWN$ is always above the threshold drawn according to the distribution $p_{\vcmp} = [0.8, 0.2]$, reaching the cap of almost 60\% ($\sim$ 8 mini-batches) towards the end. Additionally, in Figure \ref{fig:gridslope_baselines_comparison} we empirically motivate the choice of the convenient baseline $b = - \var (H_\tau)$. No advantage derives from the use of the $\var$ baseline; in fact, it leads to a slightly higher variance, as depicted in the right plot, with the mean of the gradients of the last layer of the policy, i.e. the \emph{mean actions} $\bm{\mu}_{\vtheta}(\bm{s})$ one.

\subsection{On the Value of the Percentile}
\label{sec:experiments_alpha_sensitivity}
In this section, we consider repeatedly training MEMENTO with different values of $\alpha$ in the GridWorld with Slope domain, and we compare the resulting exploration performance $\mathcal{E}_{\vcmp}^1$ as before. In Figure~\ref{fig:gridslope_alpha}, we can see that the lower $\alpha$ we choose, the more we prioritize GWN (right bar for every $\alpha$) at the expense of GWS (left bar). Note that this trend carries on with increasing $\alpha$, ending in the values of Figures~\ref{fig:gridslope_exploration_south},~\ref{fig:gridslope_exploration_north}. The reason for this behavior is quite straightforward, the smaller is $\alpha$, the larger is the share of trajectories from the adverse configuration (GWN) ending up in the percentile at first, and thus the more GWN affects the policy update (see the gradient in~\eqref{eq:policy_gradient_estimator}). 
\emph{Note that the value of the percentile $\alpha$ should not be intended as a hyper-parameter to tune via trial and error, but rather as a parameter to select the desired risk profile of the algorithm.}
Indeed, there is not a way to say which of the outcomes in Figure~\ref{fig:gridslope_alpha} is preferable, as they are all reasonable trade-offs between the average and worst-case performance, which might be suited for specific applications.
For the sake of consistency, in every experiment of our analysis we report results with a value of $\alpha$ that matches the sampling probability of the worst-case configuration, but similar arguments could be made for different choices of $\alpha$.
% One might ask how much the dimension of the percentile $\alpha$ affects the results. In Figure \ref{fig:gridslope_alpha} we report a comparison on both the configurations $GWN$ and $GWS$. The trade-off is plainly visible: a higher $\alpha$ positively impacts the exploration in $GWS$, due to the presence of more mini-batches with its own trajectories, with the drawback of a worse performance on the \emph{adversarial} $GWN$, and vice-versa. 

\subsection{RL with a General Exploration Strategy}
\label{sec:experiments_rl_illustrative}
%In this section, we illustrate how beneficial is the pre-trained exploration strategy to deal with any RL problem one could specify in the GridWorld with Slope class.
To assess the benefit of the pre-trained strategy, we design a family of MDPs $\cmp^R$, where $\cmp \in \{\text{GWS},\text{GWN}\}$, and $R$ is any sparse reward function that gives 1 when the agent reaches the area nearby a random goal location and 0 otherwise. On this family, we compare the performance achieved by TRPO~\citep{schulman2015trust} with different initializations: The exploration strategies learned (as in Section~\ref{sec:experiments_learning_to_explore_illlustrative}) by MEMENTO ($\alpha = 0.2$) and Neutral ($\alpha=1$), or a randomly initialized policy (Random). These three variations are evaluated in terms of their average return $\mathcal{J}_{\cmp^R}$, which is defined in~\eqref{eq:rl_objective}, over 50 randomly generated goal locations (Figure~\ref{fig:gridslope_sampled_goals}).
As expected, the performance of TRPO with Neutral is competitive in the GWS configuration (Figure~\ref{fig:gridslope_rl}), but it falls sharply in the GWN configuration, where it is not significantly better than TRPO with Random. Instead, the performance of TRPO with MEMENTO is strong on both GWS and GWN. Despite the simplicity of the domain, solving an RL problem in GWN with an adverse goal location is far-fetched for both a random initialization and a na\"ive solution to the reward-free exploration over multiple environments.
% We now illustrate how a learning agent can benefit from an exploration policy learned by MEMENTO in a sparse-reward RL setting, defined over the same class of environments. Especially, we compare the performance achieved by TRPO \cite{schulman2015trust} initialized with a MEMENTO policy \wrt TRPO initialized with a \emph{risk-neutral} policy and TRPO starting from scratch, i.e. with a randomly initialized policy. We consider the two configurations $GWS$ and $GWN$ and for each of them we make an evaluation in terms of average return on a series of sparse-reward RL tasks. In particular, we run 54 experiments, each one with a different randomly sampled goal location (see Figure \ref{fig:gridslope_sampled_goals}): the reward is 1 in the states having Euclidean distance to the goal lower than 0.1, while it is zero in all the remaining state space. As we show in Figure \ref{fig:gridslope_rl}, the MEMENTO initialization leads to a drastically better result in the \emph{adversarial} configuration $GWN$, while retaining a good performance in $GWS$. Notably, the \emph{risk-neutral} approach in $GWN$ is even comparable with the random initialization, probably because highly biased towards the south-slope configuration.

\input{contents/figures/multigrid_ant}
\subsection{Scaling to Larger Classes of Environments}
\label{sec:experiments_scalability_class}
In this section, we consider a class $\vcmp$ composed of ten different configurations of the continuous gridworlds presented in Section~\ref{sec:experiments_learning_to_explore_illlustrative} (including the GWN as the worst-case configuration) which we call the \emph{MultiGrid} domain. As before, we compare MEMENTO ($\alpha = 0.1$) and Neutral ($\alpha=1$) on the exploration performance $\mathcal{E}_{\vcmp}^{1}$ achieved by the optimal strategy, in this case considering a uniformly distributed $p_{\vcmp}$. While the average performance of Neutral is slightly higher across the class (Figure~\ref{fig:multigrid} left, left bar), MEMENTO still has a decisive advantage in the worst-case configuration (Figure~\ref{fig:multigrid} left, right bar). Just as in Section~\ref{sec:experiments_rl_illustrative}, this advantage transfer to RL, where we compare the average return $\mathcal{J}_{\cmp^R}$ achieved by TRPO with MEMENTO, Neutral, and Random initializations over 50 random goal locations in the GWN configuration (Figure~\ref{fig:multigrid} right). \emph{Whereas in the following sections we will only consider classes of two environments, this experiment shows that the arguments made for small classes of environments can easily generalize to larger classes.}
% In this section, we extend the previous analysis by assessing the capability of MEMENTO to scale to a larger number of environments. Especially, we consider a set of 10 GridWorld environments. The \emph{adversarial} configuration is the same as in Section \ref{subsec:risk_averse}, i.e. $GWN$, while the remaining 9 environments are characterized by different slopes (towards south, east, south-east) or by no slope at all, so that their exploration is not completely straightforward, but still easier than the adversarial one.
% Also in this case, in Figure \ref{fig:multigrid} we show the performance of MEMENTO compared to the risk-neutral approach. More precisely, the comparison is made in the \emph{adversarial configuration} (Figure \ref{fig:multigrid_exploration_worst}) and in the \emph{multiple configurations} scenario (Figure \ref{fig:multigrid_exploration_all}). In this last case, each environment is sampled with $p_{\cmp} = 0.1$. Although the difference is not as conspicuous as in the \emph{2-environments} experiment, MEMENTO still has a decisive advantage in terms of exploration in the difficult setting, while retaining an optimal performance in the multi-environment one.
% We report in Figure~\ref{fig:multigrid_rl} the RL analysis, carried out as in Section \ref{subsec:risk_averse}. We considered the same goal locations of Figure~\ref{fig:gridslope_sampled_goals}, randomly sampled in the \emph{adversarial} configuration. Even with 10 environments, different in geometrical structure and type of slope, the MEMENTO initialization leads to better performance.

\subsection{Scaling to Increasing Dimensions}
\label{sec:experiments_scalability_dimension}
In this section, we consider a class $\vcmp$ consisting of two Ant environments, with 29D states and 8D actions. In the first, sampled with probability $p_{\cmp_1} = 0.8$, the Ant faces a wide descending staircase (\emph{Ant Stairs Down}). In the second, the Ant faces a narrow ascending staircase (\emph{Ant Stairs Up}, sampled with probability $p_{\cmp_2} = 0.2$), which is significantly harder to explore than the former. In the mold of the gridworlds in Section~\ref{sec:experiments_learning_to_explore_illlustrative}, these two configurations are specifically designed to create an imbalance in the class. As in Section~\ref{sec:experiments_learning_to_explore_illlustrative}, we compare MEMENTO ($\alpha = 0.2$) against Neutral ($\alpha = 1$) on the exploration performance $\mathcal{E}_{\vcmp}^{1}$ achieved after 500 epochs. MEMENTO fares slightly better than Neutral both in the worst-case configuration (Figure~\ref{fig:ant} left, right bar) and, surprisingly, in the easier one (Figure~\ref{fig:ant} left, left bar).\footnote{Note that this would not happen in general, as we expect MEMENTO to be better in the worst-case but worse on average. Apparently, the percentile objective positively biases the average performance in this setting.}
Then, we design a set of incrementally challenging sparse-rewards RL tasks in the \emph{Ant Stairs Up}, which give reward 1 upon reaching a certain step of the staircase. Also in this setting, TRPO with Memento initialization outperforms TRPO with Neutral and Random in terms of the average return $\mathcal{J}_{\cmp^R}$ (Figure~\ref{fig:ant} right). Note that these sparse-reward continuous control tasks are particularly arduous: TRPO with Neutral and Random barely learns anything, while even TRPO with MEMENTO does not handily reach the optimal average return (1). %especially in the tasks associated to the upper steps of the staircase.

\input{contents/figures/meta}
\subsection{Scaling to Visual Inputs}
\label{sec:experiments_scalability_vision}
In this section, we consider a class $\vcmp$ of two partially-observable MiniGrid~\citep{chevalier2018minimalistic} environments, in which the observation is a 147D image of the agent's field of view. 
In Figure~\ref{fig:minigrid_visualization}, we provide a visualization of the domain: The easier configuration (EasyG, left) is sampled with probability $p_{\cmp_1} = 0.8$, the adverse configuration (AdvG, right) is sampled with probability $p_{\cmp_2} = 0.2$. Two factors make the AdvG more challenging to explore, which are the presence of a door at the top-left of the grid, and reversing the effect of agent's movements (\eg the agent goes backward when it tries to go forward). 
Whereas in all the previous experiments we estimated the entropy on the raw input features, visual inputs require a wiser choice of a metric. As proposed in~\citep{seo2021state}, we process the observations through a random encoder before computing the entropy estimate in~\eqref{eq:knn_entropy_estimator}, while keeping everything else as in Algorithm~\ref{alg:memento}. We run this slightly modified version of MEMENTO ($\alpha = 0.2$) and Neutral ($\alpha = 1$) for 300 epochs. Then, we compare TRPO with the learned initializations (as well as Random) on sparse-reward tasks defined upon the class. As in previous settings, TRPO with MEMENTO results slightly worse than TRPO with Neutral in the easier configuration (Figure~\ref{fig:minigrid}, left), but significantly better in the worst-case (Figure~\ref{fig:minigrid}, right). Notably, TRPO from scratch struggles to learn the tasks, especially in the AdvG (Figure~\ref{fig:minigrid}, right).
\emph{Although the MiniGrid domain is extremely simple from a vision standpoint, we note that the same architecture can be employed in more challenging scenarios~\citep{seo2021state}, while the focus of this experiment is the combination between visual inputs and multiple environments.}

\subsection{Comparison with Meta-RL}
\label{sec:experiments_meta}
In this section, we compare our approach against meta-training a policy with MAML~\citep{finn2017model} on the same \emph{GridWorld with Slope} ($p_{\vcmp} = [0.8, 0.2]$) and \emph{MultiGrid} (uniformly distributed $p_{\vcmp}$) domains that we have previously presented. 
Especially, we consider two relevant baselines. The first is MAML+R, to which we provide full access to the tasks (\ie rewards) during meta-training. Note that this gives MAML+R an edge over MEMENTO, which operates reward-free training. The second is MAML+DIAYN~\citep{gupta2018unsupervised}, which operates unsupervised meta-training through an intrinsic reward function learned with DIAYN~\citep{eysenbach2018diversity}.
As in previous sections, we consider the average return $\mathcal{J}_{\cmp^R}$ achieved by TRPO initialized with the exploration strategy learned by MEMENTO or the meta-policy learned by MAML+R and MAML+DIAYN. TRPO with MEMENTO fares clearly better than TRPO with the meta-policies in all the configurations (Figures~\ref{fig:maml_gridslope}, \ref{fig:maml_multigrid}). Even if it works fine in fast adaptation (see Appendix~\ref{apx:meta_experiments_details}), \emph{MAML struggles to encode the diversity of task distribution into a single meta-policy and to deal with the most adverse tasks in the long run.} Moreover, DIAYN does not specifically handle multiple environments, and it fails to cope with the larger \emph{MultiGrid} class.
%(see Appendix~\ref{apx:meta_experiments_details}).

==> contents/sections/introduction.tex <==
% RL limitation
The typical Reinforcement Learning~\citep[RL,][]{sutton2018reinforcement} setting involves a learning agent interacting with an environment in order to maximize a reward signal. In principle, the reward signal is a given and perfectly encodes the task. In practice, the reward is usually hand-crafted, and designing it to make the agent learn a desirable behavior is often a huge challenge. This poses a serious roadblock on the way of autonomous learning, as any task requires a costly and specific formulation, while the synergy between solving one RL problem and another is very limited.
% Reward-free RL
To address this crucial limitation, \citet{jin2020rewardfree} have formulated the \emph{reward-free} RL problem. In this setting, the agent is tasked with mastering an environment without rewards, so that the knowledge it acquires can be eventually deployed to solve any RL problem one could specify in this same environment. \emph{Mastering} the environment has been formulated in (i) \emph{learning to model} its transition dynamics up to a convenient confidence \citep{jin2020rewardfree,tarbouriech2020active}, or (ii) \emph{learning to explore} it with a general, task-agnostic, strategy~\citep{hazan2019maxent}. Although they overcome the reliance on a reward function, all of the previous solutions to reward-free RL are still severely environment-specific.

% General problem
In this work, we aim to push the generality of reward-free learning even further by addressing the problem of \emph{learning to explore multiple environments} with a single exploration strategy. In this setting, the agent faces a class of reward-free environments that belong to the same domain but differ in their transition dynamics. At each turn of the learning process, the agent is drawn into an environment within the class, where it can interact for a finite number of steps before facing another turn. The process carries on sequentially for a finite number of turns. The ultimate goal of the agent is to learn an exploration strategy that helps to solve any subsequent RL task specified over the class.
%reducing the burden on manual reward design while improving learning efficiency over RL from scratch.

% Our contributions
Our contribution to the problem is three-fold: (c1) We frame it into a tractable \emph{formulation} (Section~\ref{sec:problem}), (c2) we propose a \emph{methodology} to address it (Section~\ref{sec:method}), for which (c3) we provide a thorough \emph{empirical} evaluation (Section~\ref{sec:experiments}).
First, we extend a reward-free objective meant for environment-specific exploration, which is the \emph{Maximum State Visitation Entropy}~\citep[MSVE,][]{hazan2019maxent}. The underlying intuition is that a general exploration strategy has to visit with high probability any state where the agent might be rewarded in a subsequent RL task. When dealing with multiple environments, this becomes a \emph{multi-objective} problem, as one could establish any combination of preferences over the environments. In this work, instead of na\"ively optimizing the mean of the state visitation entropy across the class, we consider its Conditional Value-at-Risk~\citep[CVaR,][]{rockafellar2000optimization} to prioritize performance in particularly rare or adverse environments. 
We propose a policy gradient algorithm~\citep{deisenroth2013survey}, \emph{Multiple Environments Maximum ENTropy Optimization} (MEMENTO), to optimize the learning objective via mere interactions with the class of environments. As in recent works~\citep{mutti2020policy,anonymous2021unsupervised,seo2021state}, the algorithm employs non-parametric methods to deal with state entropy estimation in continuous and high-dimensional environments. Then, it leverages these estimated values to optimize the CVaR of the entropy by following its policy gradient~\citep{tamar2015optimizing}.
Finally, we provide an experimental analysis of the proposed method in a two-stage setting. First, we show that it is effective in training general exploration strategies over classes of continuous and high-dimensional environments without rewards. Second, we test the obtained exploration strategies as initialization for a number of RL tasks defined over the same class. Notably, the trained exploration strategy allows us to solve sparse-rewards tasks that are impractical to learn from scratch, while being robust to the most unfavorable environment thanks to the CVaR objective.
Related works are in Section~\ref{sec:related_work}, a preliminary theoretical analysis is in Appendix~\ref{sec:theory}, the proofs of the theorems are in Appendix~\ref{apx:proofs}. 
%The implementation of MEMENTO can be found at \url{https://github.com/muttimirco/memento}.


==> contents/sections/method.tex <==
In this section, we present an algorithm, called \emph{Multiple Environments Maximum ENTropy Optimization} (MEMENTO), to optimize the exploration objective in~\eqref{eq:exp_risk_averse}
through mediated interactions with a class of continuous environments. 

MEMENTO operates as a typical policy gradient approach \citep{deisenroth2013survey}. It directly searches for an optimal policy by navigating a set of parametric differentiable policies $\Pi_{\Theta} := \lbrace \pi_{\vtheta} : \vtheta \in \Theta \subseteq \reals^n \rbrace$. It does so by repeatedly updating the policy parameters $\vtheta$ in the gradient direction, until a stationary point is reached. This update has the form
\begin{equation*}
    \vtheta ' = \vtheta + \beta \nabla_{\vtheta} \mathcal{E}_{\vcmp}^{\alpha} (\pi_{\vtheta}),
\end{equation*}
where $\beta$ is a learning rate, and $\nabla_{\vtheta} \mathcal{E}_{\vcmp}^{\alpha} (\pi_{\vtheta})$ is the gradient of~\eqref{eq:exp_risk_averse} \wrt $\vtheta$. The following proposition provides the formula of $\nabla_{\vtheta} \mathcal{E}_{\vcmp}^{\alpha} (\pi_{\vtheta})$. The derivation follows closely the one in~\citep[][Proposition 1]{tamar2015optimizing}, which we have adapted to our objective function of interest~\eqref{eq:exp_risk_averse}.
\begin{restatable}[]{prop}{cvarPolicyGradient}
The policy gradient of the exploration objective $\mathcal{E}_{\vcmp}^{\alpha} (\pi_{\vtheta})$ \wrt $\vtheta$ is given by
\begin{align}
    \nabla_{\vtheta} & \mathcal{E}_{\vcmp}^{\alpha} (\pi_{\vtheta}) =
    \EV_{\substack{\cmp \sim p_{\vcmp} \\ \tau \sim p_{\pi_{\vtheta},\cmp}}} 
    \bigg[ \bigg( \sum_{t = 0}^{T - 1} \nabla_{\vtheta} \log \pi_{\vtheta} (a_{t,\tau}|s_{t,\tau}) \bigg) \nonumber \\
    &\times \bigg( H_{\tau} - \var (H_\tau) \bigg) \bigg| H_{\tau} \leq \var (H_\tau) \bigg].
\end{align}
\label{prop:cvar_policy_gradient}
\end{restatable}
However, in this work we do not assume full knowledge of the class of CMPs $\vcmp$, and the expected value in Proposition~\ref{prop:cvar_policy_gradient} cannot be computed without having access to $p_{\vcmp}$ and $p_{\pi_{\vtheta}, \cmp}$. Instead, MEMENTO computes the policy update via a Monte Carlo estimation of $\nabla_{\vtheta} \mathcal{E}_{\vcmp}^{\alpha}$ from the sampled interactions $\lbrace (\cmp_i, \tau_i) \rbrace_{i = 1}^N$ with the class of environments $\vcmp$. The policy gradient estimate itself relies on a Monte Carlo estimate of each entropy value $H_{\tau_i}$ from $\tau_i$, and a Monte Carlo estimate of $\var (H_\tau)$ given the estimated $\lbrace H_{\tau_i} \rbrace_{i = 1}^N$. The following paragraphs describe how these estimates are carried out, while Algorithm~\ref{alg:memento} provides the pseudocode of MEMENTO. Additional details and implementation choices can be found in Appendix~\ref{apx:algorithm}.
\begin{algorithm}[t]
\caption{MEMENTO}
\label{alg:memento}
    \textbf{Input}: percentile $\alpha$, learning rate $\beta$\\
    \textbf{Output}: policy $\pi_{\bm{\theta}}$
    \begin{algorithmic}[1] %[1] enables line numbers
        \STATE initialize $\vtheta$
        \FOR{epoch $= 0,1,\ldots$, until convergence}
        \FOR{$i = 1,2,\ldots, N$}
        \STATE{sample an environment $\mathcal{M}_i \sim p_{\vcmp}$}
        \STATE sample a trajectory $\tau_i \sim p_{\pi_{\vtheta}, \cmp_i}$
        \STATE estimate $H_{\tau_i}$ with~\eqref{eq:knn_entropy_estimator}
        \ENDFOR
        \STATE estimate $\var (H_\tau)$ with~\eqref{eq:var_estimator}
        \STATE estimate $\nabla_{\vtheta} \mathcal{E}_{\vcmp}^{\alpha} (\pi_{\vtheta})$ with~\eqref{eq:policy_gradient_estimator}
        \STATE update parameters $\vtheta \gets \vtheta + \beta \widehat{\nabla}_{\vtheta} \mathcal{E}_{\cmp}^{\alpha} (\pi_{\vtheta})$
        \ENDFOR
    \end{algorithmic}
\end{algorithm}

\paragraph{Entropy Estimation}
We would like to compute the entropy $H_{\tau_i}$ of the state visitation frequencies $d_{\tau_i}$ from a single realization $\lbrace s_{t,\tau_i} \rbrace_{t=0}^{T - 1} \subset \tau_i$. This estimation is notoriously challenging when the state space is continuous and high-dimensional $\sspace \subseteq \reals^p$. Taking inspiration from recent works pursuing the MSVE objective~\citep{mutti2020policy,anonymous2021unsupervised,seo2021state}, we employ a principled $k$-Nearest Neighbors ($k$-NN) entropy estimator~\citep{singh2003nearest} of the form
\begin{equation}
    \widehat{H}_{\tau_i} \propto - \frac{1}{T} \sum_{t = 0}^{T - 1}
    \log \frac{k \ \Gamma (\frac{p}{2} + 1)}{T \ \big\| s_{t,\tau_i} - s^{k\text{-NN}}_{t, \tau_i} \big\|^p \ \pi^{\frac{p}{2}}},
    \label{eq:knn_entropy_estimator}
\end{equation}
where $\Gamma$ is the Gamma function, $\|\cdot\|$ is the Euclidean distance, and $s_{t, \tau_i}^{k\text{-NN}} \in \tau_i$ is the $k$-nearest neighbor of $s_{t,\tau_i}$. The intuition behind the estimator in $\eqref{eq:knn_entropy_estimator}$ is straightforward: We can suppose the state visitation frequencies $d_{\tau_i}$ to have a high entropy as long as the average distance between any encountered state and its $k$-NN is large. Despite its simplicity, a Euclidean metric suffices to get reliable entropy estimates in continuous control domains~\citep{mutti2020policy}.

\paragraph{VaR Estimation and Baseline}
The last missing piece to get a Monte Carlo estimate of the policy gradient $\nabla_{\vtheta} \mathcal{E}_{\vcmp}^\alpha$ is the value of $\var (H_\tau)$. Being $H_{[1]}, \ldots, H_{[N]}$ the order statistics out of the estimated values $\lbrace \widehat{H}_{\tau_i} \rbrace_{i = 1}^N$, we can na\"ively estimate the VaR as
\begin{equation}
    \evar (H_\tau) = H_{[\lceil \alpha N \rceil]}.
    \label{eq:var_estimator}
\end{equation}
Albeit asymptotically unbiased, the VaR estimator in~\eqref{eq:var_estimator} is known to suffer from a large variance in finite sample regimes~\citep{kolla2019concentration}, which is aggravated by the error in the upstream entropy estimates, which provide the order statistics.
This variance is mostly harmless when we use the estimate to filter out entropy values beyond the $\alpha$\%, \ie the condition $H_\tau \leq \var (H_\tau)$ in Proposition~\ref{prop:cvar_policy_gradient}. Instead, its impact is significant when we subtract it from the values within the $\alpha$\%, \ie the term $H_\tau - \var (H_\tau)$ in Proposition~\ref{prop:cvar_policy_gradient}. 
To mitigate this issue, we consider a convenient baseline $b = - \var (H_\tau)$ to be subtracted from the latter, which gives the Monte Carlo policy gradient estimator
\begin{equation}
    \widehat{\nabla}_{\vtheta} \mathcal{E}_{\vcmp}^\alpha (\pi_{\vtheta})
    = \sum_{i = 1}^N  f_{\tau_i} \ \widehat{H}_{\tau_i} \ \ind (\widehat{H}_{\tau_i} \leq \evar (H_\tau)),
    \label{eq:policy_gradient_estimator}
\end{equation}
where $f_{\tau_i} = \sum_{t = 0}^{T - 1} \nabla_{\vtheta} \log \pi_{\vtheta} (a_{t,\tau_i}|s_{t,\tau_i})$. Notably, the baseline $b$ trades off a lower estimation error for a slight additional bias in the estimation~\eqref{eq:policy_gradient_estimator}. We found that this baseline leads to empirically good results and we provide some theoretical corroboration over its benefits in Appendix~\ref{apx:algorithm_baseline}.


==> contents/sections/preliminaries.tex <==
In this section, we report background and notation. A vector $\bm{v}$ is denoted in bold, and $v_i$ stands for its $i$-th entry.

\paragraph{Probability and Percentiles}
Let $X$ be a random variable distributed according to a cumulative density function (cdf) $F_X (x) = Pr (X \leq x)$. We denote with $\EV [X]$, $\Var [X]$ the expected value and the variance of $X$ respectively.
Let $\alpha \in (0, 1)$ be a confidence level, we call the $\alpha$-percentile (shortened to $\alpha$\%) of the variable $X$ its Value-at-Risk (VaR), which is defined as
$$
    \var (X) = \inf \big\lbrace x \;|\; F_X (x) \geq \alpha \big\rbrace.
$$
Analogously, we call the mean of this same $\alpha$-percentile the Conditional Value-at-Risk (CVaR) of $X$,
$$
    \cvar (X) = \EV \big[ X \;|\; X \leq \var (X) \big].
$$

\paragraph{Markov Decision Processes}
A Controlled Markov Process (CMP) is a tuple $\mathcal{M} := (\sspace, \aspace, P, D)$, where $\sspace$ is the state space, $\aspace$ is the action space, the transition model $P(s' | a, s)$ denotes the conditional probability of reaching state $s' \in \sspace$ when selecting action $a \in \aspace$ in state $s \in \sspace$, and $D$ is the initial state distribution.
The behavior of an agent is described by a policy $\pi (a | s)$, which defines the probability of taking acion $a \in \aspace$ in $s \in \sspace$. Let $\Pi$ be the set of all the stationary policies.
Executing a policy $\pi \in \Pi$ in a CMP over $T$ steps generates a trajectory $\tau = (s_{0,\tau}, a_{0,\tau}, \ldots, a_{T-2,\tau}, s_{T - 1, \tau})$ with probability
$$
    p_{\pi, \cmp} (\tau) = D(s_{0, \tau}) \prod^{T - 1}_{t = 0} \pi(a_{t,\tau} | s_{t,\tau}) P (s_{t+1,\tau}| s_{t,\tau}, a_{t,\tau}).
$$
We denote the state-visitation frequencies induced by $\tau$ with $ d_\tau (s) = \frac{1}{T} \sum_{t=0}^{T-1} \ind (s_{t,\tau} = s)$, and we call $d_\pi^{\cmp} = \EV_{\tau \sim p_{\pi, \cmp}} [d_{\tau}]$ the marginal state distribution. We define the differential entropy~\citep{shannon1948entropy} of $d_\tau$ as 
$$ 
	H (d_\tau) = - \int_\sspace d_\tau (s) \log d_{\tau} (s) \de s.
$$
For simplicity, we will write $H (d_\tau)$ as a random variable $H_\tau \sim \delta (h - H(d_\tau)) p_{\pi, \cmp} (\tau)$, where $\delta(h)$ is a Dirac delta.

By coupling a CMP $\cmp$ with a reward function $R$ we obtain a Markov Decision Process~\citep[MDP,][]{puterman2014markov} $\cmp^R := \cmp \cup R$. Let $R(s, a)$ be the expected immediate reward when taking $a \in \aspace$ in $s \in \sspace$ and let $R(\tau) = \sum_{t=0}^{T -1} R (s_{t, \tau})$, the \emph{performance} of a policy $\pi$ over the MDP $\cmp^R$ is defined as
\begin{equation}
    \mathcal{J}_{\cmp^R} (\pi) = \EV_{\tau \sim p_{\pi,\cmp}} \big[ R (\tau) \big].
    \label{eq:rl_objective}
\end{equation}
The goal of reinforcement learning~\cite{sutton2018reinforcement} is to find an optimal policy $\pi^*_{\mathcal{J}} \in \arg \max \mathcal{J}_{\cmp^R} (\pi)$ through sampled interactions with an unknown MDP $\cmp^R$.


==> contents/sections/problem.tex <==
\input{contents/figures/problem}
%In this section, we present the objective for \emph{learning to explore multiple environments} with a unique general strategy.
Let $\vcmp = \{\cmp_1, \ldots, \cmp_{I}\}$ be a class of unknown CMPs, in which every  element $\cmp_i = (\sspace, \aspace, P_i, D)$ has a specific transition model $P_i$, while $\sspace, \aspace, D$ are homogeneous across the class. At each turn, the agent is able to interact with a single environment $\cmp \in \vcmp$. The selection of the environment to interact with is mediated by a distribution $p_{\vcmp}$ over $\vcmp$, outside the control of the agent. The aim of the agent is to learn an exploration strategy that is general across all the MDPs $\cmp^R$ one can build upon $\vcmp$. In a single-environment setting, this problem has been assimilated to learning a policy that maximizes the entropy of the induced state visitation frequencies~\citep{hazan2019maxent,lee2019smm,mutti2020policy}. One can straightforwardly extend the objective to multiple environments by considering the expectation over the class of CMPs,
$
    \mathcal{E}_{\vcmp} (\pi) = \EV_{\substack{\cmp \sim p_{\vcmp} \\ \tau \sim p_{\pi, \cmp}}} \big[ H_{\tau} \big],
    %\label{eq:exp_risk_neutral}
$
where the usual entropy objective over the single environment $\cmp_i$ can be easily recovered by setting $p_{\cmp_i} = 1$.
However, this objective function does not account for the tail behavior of $H_\tau$, \ie for the exploration performance in environments of $\vcmp$ that are rare or particularly unfavorable. This is decidedly undesirable as the agent may be tasked with an MDP built upon one of these adverse environments in the subsequent RL phase, where even an optimal strategy \wrt $\mathcal{E}_{\vcmp} (\pi)$ may fail to provide sufficient exploration. To overcome this limitation, we look for a more nuanced exploration objective that balances the expected performance with the sensitivity to the tail behavior. By taking inspiration from the risk-averse optimization literature~\citep{rockafellar2000optimization}, we consider the CVaR of the state visitation entropy induced by $\pi$ over $\vcmp$,
\begin{align}
    \mathcal{E}_{\vcmp}^\alpha (\pi) &= \cvar (H_\tau) \nonumber \\
    &= \EV_{\substack{\cmp \sim p_{\vcmp} \\ \tau \sim p_{\pi, \cmp}}} \big[ H_{\tau} \;|\; H_{\tau} \leq \var (H_\tau) \big],
    \label{eq:exp_risk_averse}    
\end{align}
where $\alpha$ is a confidence level and $\mathcal{E}_{\vcmp}^1 (\pi) := \mathcal{E}_{\vcmp} (\pi)$. The lower we set the value of $\alpha$, the more we hedge against the possibility of a bad exploration outcome in some $\cmp \in \vcmp$.
In the following sections, we propose a method to effectively learn a policy $\pi^*_{\mathcal{E}} \in \arg \max \mathcal{E}_{\vcmp}^\alpha (\pi)$ through mere interactions with $\vcmp$, and we show how this serves as a pre-training for RL (the full process is depicted in Figure~\ref{fig:problem}).

==> contents/sections/related_work.tex <==
Our work lies at the intersection of reward-free exploration, robust and risk-averse RL, and meta-RL. 
%(Figure~\ref{fig:related_work}).
%\begin{wrapfigure}{R}{0.50\textwidth}
%\vspace{-0.5cm}
%\begin{minipage}{0.49\textwidth}
%\input{contents/figures/related_work}
%\end{minipage}
%\end{wrapfigure}

% Entropy Maximization
The literature that relates the most with our work is the one pursuing a \emph{MSVE objective} in reward-free settings. Some methods~\citep{hazan2019maxent,lee2019smm} focus on learning a mixture of policies that is collectively MSVE optimal, while other~\citep{tarbouriech2019active, mutti2020intrinsically} casts the MSVE as a dual (or surrogate) linear program in tabular settings. Successive works tackle MSVE at scale with non-parametric entropy estimation~\citep{mutti2020policy,anonymous2021unsupervised, liu2021aps, yarats2021reinforcement, seo2021state}, or introduce variations to the entropy objective, such as geometry-awareness~\citep{guo2021geometric} and R\'enyi generalization~\citep{zhang2020exploration}. To the best of our knowledge, all existing solutions are environment-specific and do not directly address multiple environments.

% Robust RL and risk-aversion
Previous work considered \emph{CVaR optimization} in RL, either to learn a policy that is averse to the risk induced by the volatility of returns~\citep{tamar2015optimizing,chow2014algorithms} or by changes in the environment dynamics~\citep[\eg][]{rajeswaran2016epopt}. Here we account for a different source of risk, which is the one of running into a particularly unfavorable environment for the trained exploration strategy.

% Meta RL
Finally, the two-stage learning setting we address has clear connections with the \emph{meta-RL} problem setting \citep{finn2017model}, in which we would call meta-training the reward-free phase, and meta-testing the subsequent RL tasks. While some methods target exploration in meta-RL \citep[\eg][]{xu2018meta, gupta2018maesn, zintgraf2019varibad}, they usually assume access to rewards during meta-training, with the notable exception of~\citep{gupta2018unsupervised}. To the best of our knowledge, none of the existing works combine reward-free meta-training with a multiple-environments setting.

==> submission/contents/figures/antmaze_env_apx.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{contents/images/antmaze_down_stairs.png}
        \caption{Ant Stairs Down}
        \label{fig:ant_stairs_down}
    \end{subfigure}
    \hspace{3em}
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{contents/images/antmaze_up_stairs.png}
        \caption{Ant Stairs Up}
        \label{fig:ant_stairs_up}
    \end{subfigure}
    \caption{Illustration of the \emph{Ant Stairs} domain. We show a render of the \emph{Ant Stairs Down} environment \textbf{(a)} and of the adverse \emph{Ant Stairs Up} environment \textbf{(b)}.}
    \label{fig:antmaze_env_apx}
\end{figure}

==> submission/contents/figures/baseline.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[scale=1]{contents/plot_files/img/gridslope_baseline2.pdf}
    \caption{Comparison of the exploration performance $\mathcal{E}_{\vcmp}^{0.35}$ (left) and sampled gradients of the policy mean (right) achieved by $\alpha$MEPOL ($\alpha=0.35$) with and without the baseline $b = - \var (H_\tau)$ in the policy gradient estimation \eqref{eq:policy_gradient_estimator}. We provide 95\% c.i. over 4 runs.}
    \label{fig:gridslope_baseline}
\end{figure*}

==> submission/contents/figures/counterexample.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/counterexample_all.pdf}
        \caption{$p_{\vcmp} = [0.8, 0.2]$}
        \label{fig:counterexample_all}
    \end{subfigure}
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/counterexample_env_1.pdf}
        \caption{$p_{\vcmp} = [1, 0]$}
        \label{fig:counterexample_env_1}
    \end{subfigure}
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/counterexample_env_2.pdf}
        \caption{$p_{\vcmp} = [0, 1]$}
        \label{fig:counterexample_env_2}
    \end{subfigure}
    \caption{Comparison of the exploration performance $\mathcal{E}_{\vcmp}^1$ obtained by $\alpha$MEPOL ($\alpha = 0.35$) and MEPOL in the \emph{GridWorld Counterexample} domain. The polices are trained (50 epochs, $8 \times 10^4$ samples per epoch) on the configuration \textbf{(a)} and tested on \textbf{(a, b, c)}. We provide 95\% c.i. over 4 runs.}
    \label{fig:counterexample}
\end{figure*}

==> submission/contents/figures/counterexample2.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[t]{0.2\textwidth}
        \centering
        \includegraphics[scale=0.2, valign=b]{contents/images/minigrid_unlock}
        \caption{Unlock-v0}
        \label{fig:counterexample_unlock}
    \end{subfigure}
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[scale=0.45, valign=b]{contents/images/minigrid_obstructed_maze}
        \caption{ObstructedMaze-2Dlhb-v0}
        \label{fig:counterexample_obstructed}
    \end{subfigure}
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[scale=1, valign=b]{contents/plot_files/img/minigrid_unlock_obstructed.pdf}
        \caption{$p_{\vcmp} = [0.8, 0.2]$}
        \label{fig:counterexample_minigrid}
    \end{subfigure}
    \caption{Comparison of the exploration performance $\mathcal{E}_{\vcmp}^{0.2}$ obtained by $\alpha$MEPOL ($\alpha = 0.2$) and MEPOL \textbf{(c)} in a \emph{MiniGrid} domain with the configurations \emph{Unlock-v0} \textbf{(a)} and \emph{ObstructedMaze-2Dlhb-v0} \textbf{(b)}. We provide 95\% c.i. over 8 runs.}
    \label{fig:counterexample2}
\end{figure*}

==> submission/contents/figures/gridslope.tex <==
\begin{figure*}[t]
    \begin{subfigure}[t]{0.34\textwidth}
        \centering
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/gridslope_illustration.pdf}
        \vspace{5pt}
        \caption{GridWorld with Slope}
        \label{fig:gridslope_illustration}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.21\textwidth}
        \centering
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/gridslope_exploration_all.pdf}
        \vspace{-0.2cm}
        \caption{$p_{\vcmp} = [0.8, 0.2]$}
        \label{fig:gridslope_exploration_all}
    \end{subfigure}
    %\hfill
        \begin{subfigure}[t]{0.21\textwidth}
        \centering
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/gridslope_exploration_south.pdf}
        \vspace{-0.2cm}
        \caption{$p_{\vcmp} = [1, 0]$}
        \label{fig:gridslope_exploration_south}
    \end{subfigure}
    %\hfill
    \begin{subfigure}[t]{0.22\textwidth}
        \centering
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/gridslope_exploration_north.pdf}
        \vspace{-0.2cm}
        \caption{$p_{\vcmp} = [0, 1]$}
        \label{fig:gridslope_exploration_north}
    \end{subfigure}
    
    \vspace{0.2cm}
    \begin{subfigure}[t]{0.53\textwidth}
        \centering
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/gridslope_empirical_distribution.pdf}
        \vspace{-0.2cm}
        \caption{MEPOL (left) and $\alpha$MEPOL (right)}
        \label{fig:gridslope_empirical_distribution}
    \end{subfigure}
    %\hfill
    \begin{subfigure}[t]{0.47\textwidth}
        \centering
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/gridslope_alpha2.pdf}
        \vspace{-0.2cm}
        \caption{$\alpha$ sensitivity of $\alpha$MEPOL}
        \label{fig:gridslope_alpha}
    \end{subfigure}
%    \begin{subfigure}[t]{0.21\textwidth}
%        \centering
%        \includegraphics[scale=1, valign=t]{contents/plot_files/img/gridslope_alpha.pdf}
%        \vspace{-0.2cm}
%        \caption{$\alpha$ sensitivity}
%        \label{fig:gridslope_alpha}
%    \end{subfigure}
%    %\hfill
%    \begin{subfigure}[t]{0.235\textwidth}
%        \centering
%        \includegraphics[scale=1, valign=t]{contents/plot_files/img/gridslope_alpha_composition.pdf}
%        \vspace{-0.2cm}
%        \caption{$\alpha$\% composition}
%        \label{fig:gridslope_alpha_composition}
%    \end{subfigure}
    %\vspace{-0.2cm}
    \caption{Pre-training performance $\mathcal{E}_{\vcmp}^1$ obtained by $\alpha$MEPOL ($\alpha = 0.2$) and MEPOL in the \emph{GridWorld with Slope} domain \textbf{(a)}. The polices are trained on  \textbf{(b)} and tested on \textbf{(b, c, d)}. The dashed lines in \textbf{(c, d)} represent the optimal performance. The empirical distribution having mean in \textbf{(b)} is reported in \textbf{(e)}. The behaviour of $\alpha$MEPOL with different $\alpha$ is reported in \textbf{(f)}. For every plot, we provide 95\% c.i. over 10 runs.}
    \label{fig:gridslope_exploration}
\end{figure*}

==> submission/contents/figures/gridslope_rl.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.5\textwidth}
        \centering
        \includegraphics[scale=1]{contents/plot_files/img/gridslope_rl.pdf}
        \vspace{-0.15cm}
        \caption{Fine-tuning on GWS (left) and GWN (right)}
        \label{fig:gridslope_rl_return}
    \end{subfigure}
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[scale=1]{contents/plot_files/img/gridslope_sampled_goals.pdf}
        \vspace{-0.2cm}
        \caption{Sampled goals}
        \label{fig:gridslope_sampled_goals}
     \end{subfigure}
     %\vspace{-0.2cm}
    \caption{Fine-tuning performance $\mathcal{J}_{\cmp^R}$ as a function of learning epochs achieved by TRPO initialized with $\alpha$MEPOL ($\alpha = 0.2$), MEPOL, and random exploration strategies, when dealing with a set of RL tasks specified on the \emph{GridWorld with Slope} domain \textbf{(a)}. We provide 95\% c.i. over 50 randomly sampled goal locations \textbf{(b)}.}
    \label{fig:gridslope_rl}
\end{figure*}

==> submission/contents/figures/meta.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[scale=1]{contents/plot_files/img/legend_maml.pdf}
    
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/meta_new_param_gridslope.pdf}
        \vspace{-0.2cm}
        \caption{GridWorld with Slope: GWS (left) and GWN (right)}
        \label{fig:maml_gridslope}
    \end{subfigure}
    \hspace{0.5cm}
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/meta_new_param_multigrid.pdf}
        \vspace{-0.2cm}
        \caption{MultiGrid}
        \label{fig:maml_multigrid}
    \end{subfigure}
    % \begin{subfigure}[t]{0.24\textwidth}
    %     \centering
    %     \includegraphics[scale=0.85, valign=t]{contents/plot_files/img/maml_gridslope_adaptation.pdf}
    %     \vspace{-0.2cm}
    %     \caption{Fast Adaptation}
    %     \label{fig:maml_adaptation}
    % \end{subfigure}
    %\vspace{-0.2cm}
    \caption{Fine-tuning performance $\mathcal{J}_{\cmp^R}$ achieved by TRPO initialized with $\alpha$MEPOL ($\alpha = 0.2$ \textbf{(a)}, $\alpha=0.1$ \textbf{(b)}), a MAML+R meta-policy, and a MAML+DIAYN meta-policy, when dealing with a set of RL tasks in the \emph{GridWorld with Slope} \textbf{(a)} and the \emph{MultiGrid} \textbf{(b)} domains. We provide 95\% c.i. over 50 tasks. 
    %We illustrate the fast-adapting behavior of the MAML policy in \textbf{(c)}.
    }
    \label{fig:maml}
\end{figure*}

==> submission/contents/figures/meta_details.tex <==
\begin{figure*}[ht!]
    \centering
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[scale=1, valign=b]{contents/plot_files/img/maml_gridslope_adaptation.pdf}
        \caption{MAML: Fast Adaptation}
        \label{fig:adaptation}
    \end{subfigure}
    \begin{subfigure}[t]{0.4\textwidth}
        \centering
        \includegraphics[scale=1, valign=b]{contents/plot_files/img/diayn_discriminability.pdf}
        \caption{DIAYN: Discriminability}
        \label{fig:discriminability}
    \end{subfigure}
    \caption{We illustrate the fast-adapting behavior of MAML in the \emph{GridWorld with Slope} \textbf{(a)}, and the skills discriminability of DIAYN as a function of learning epochs \textbf{(b)}. We provide 95\% c.i. over 8 runs.}
    \label{fig:meta_details}
\end{figure*}

==> submission/contents/figures/multigrid_ant.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[scale=1]{contents/plot_files/img/legend_rl.pdf}
    
    %\centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/multigrid_exploration.pdf}
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/multigrid_rl.pdf}
        \vspace{-0.2cm}
        \caption{MultiGrid: Pre-training (left) and fine-tuning (right)}
        \label{fig:multigrid}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/antmaze_exploration.pdf}
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/antmaze_rl.pdf}
        \vspace{-0.2cm}
        \caption{Ant: Pre-training (left) and fine-tuning (right)}
        \label{fig:ant}
    \end{subfigure}
    
    \vspace{0.2cm}
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \hspace{0.5cm}
        \includegraphics[scale=0.132, valign=t]{contents/images/minigrid_easy_config.png}
        \hspace{0.8cm}
        \includegraphics[scale=0.235, valign=t]{contents/images/minigrid_adverse_config.png}
        \vspace{0.03cm}
        \caption{MiniGrid: EasyG (left) and AdvG (right)}
        \label{fig:minigrid_visualization}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[scale=1, valign=t]{contents/plot_files/img/minigrid_rl.pdf}
        \vspace{-0.2cm}
        \caption{MiniGrid: fine-tuning on EasyG (left) and AdvG (right)}
        \label{fig:minigrid}
    \end{subfigure}
    %\vspace{-0.2cm}
    \caption{Pre-training performance $\mathcal{E}^1_{\vcmp}$ (95\% c.i. over 10 runs) achieved by $\alpha$MEPOL ($\alpha=0.1$ \textbf{(a)}, $\alpha = 0.2$ \textbf{(b)}) and MEPOL in the in the \emph{MultiGrid} \textbf{(a)} and \emph{Ant} \textbf{(b)} domains.
    Fine-tuning performance $\mathcal{J}_{\cmp^R}$ (95\% c.i. over 50 tasks \textbf{(a)}, 8 tasks \textbf{(b)}, 13 tasks \textbf{(d)}) obtained by TRPO with corresponding initialization ($\alpha$MEPOL, MEPOL, Random), in the \emph{MultiGrid} \textbf{(a)}, \emph{Ant} \textbf{(b)}, and \emph{MiniGrid} \textbf{(d)} domains. \emph{MiniGrid} domains are illustrated in \textbf{(c)}.}
\end{figure*}

==> submission/contents/figures/multigrid_heatmaps_apx.tex <==
\begin{figure}[b]
    \centering
    \begin{subfigure}[b]{0.85\textwidth}
        \centering
        \includegraphics[width=\textwidth]{contents/images/multigrid_memento_heatmaps.png}
        \caption{$\alpha$MEPOL}
        \label{fig:multigrid_memento_heatmaps}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.85\textwidth}
        \centering
        \includegraphics[width=\textwidth]{contents/images/multigrid_neutral_heatmaps.png}
        \caption{MEPOL}
        \label{fig:multigrid_neutral_heatmaps}
    \end{subfigure}
    \caption{Heatmaps of the state visitations (200 trajectories) induced by the exploration policies trained with $\alpha$MEPOL ($\alpha = 0.1$) \textbf{(a)} and MEPOL \textbf{(b)} in the \emph{MultiGrid} domain.}
    \label{fig:multigrid_heatmaps}
\end{figure}

==> submission/contents/figures/old/gridslope_alpha_sensitivity.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
    \centering
    \includegraphics[width=\textwidth]{contents/plot_files/img/gridslope_percentile_dist.pdf}
    \caption{Percentile distribution}
    \label{fig:gridslope_perc_dist}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.6\textwidth}
    \centering
    \includegraphics[width=\textwidth]{contents/plot_files/img/gridslope_percentiles_comparison.pdf}
    \caption{$\alpha$ comparison}
    \label{fig:gridslope_percentiles_comparison}
    \end{subfigure}
    \caption{$\textbf{(a)}$ Percentage of mini-batches inside the $\alpha$-percentile ($\alpha = 0.35$) for each configuration throughout the training. The two dotted lines represent the quantity that one could expect if considering the distribution $p_{\vcmp} = [0.8, 0.2]$. $\textbf{(b)}$ Comparison between optimal policies trained with different value of $\alpha$. (95\% c.i. over 4 runs, $N_{traj} = 200$, $T = 400$).}
    \label{fig:alpha_sensitivity}
\end{figure*}

==> submission/contents/figures/old/gridslope_configs.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[scale=0.7]
    \draw (0,0) -- (4,0) -- (4,4) -- (0,4) -- cycle;
    \fill[yellow] (0.3,3.7) -- (0.8,3.7) -- (0.8,3.2) -- (0.3,3.2) -- cycle;
    % bottom-left
    \draw[line] (0.3,0.3) -- (0.3,1.75);
    \draw[line] (0.3,1.75) -- (1.05,1.75);
    \draw[line] (1.35,1.75) -- (1.75,1.75);
    \draw[line] (1.75,1.75) -- (1.75,1.35);
    \draw[line] (1.75,1.05) -- (1.75,0.3);
    \draw[line] (1.75,0.3) -- (0.3,0.3);
    
    % top-left
    \draw[line] (0.3,2.25) -- (0.3,3.7);
    \draw[line] (0.3,3.7) -- (1.75,3.7);
    \draw[line] (1.75,3.7) -- (1.75,2.95);
    \draw[line] (1.75,2.25) -- (1.75,2.65);
    \draw[line] (1.75,2.25) -- (1.35,2.25);
    \draw[line] (1.05,2.25) -- (0.3,2.25);
    
    % top-right
    \draw[line] (2.25,2.25) -- (2.25,2.65);
    \draw[line] (2.25,2.95) -- (2.25,3.7);
    \draw[line] (2.25,3.7) -- (3.7,3.7);
    \draw[line] (3.7,3.7) -- (3.7,2.25);
    \draw[line] (3.7,2.25) -- (2.95,2.25);
    \draw[line] (2.65,2.25) -- (2.25,2.25);
    
    % bottom-right
    \draw[line] (2.25,0.3) -- (2.25, 1.05);
    \draw[line] (2.25,1.35) -- (2.25, 1.75);
    \draw[line] (2.25,1.75) -- (2.65,1.75);
    \draw[line] (2.95,1.75) -- (3.7,1.75);
    \draw[line] (3.7,1.75) -- (3.7,0.3);
    \draw[line] (3.7,0.3) -- (2.25,0.3);
    
    % Hallways
    \draw[line] (1.05,1.75) -- (1.05,2.25);
    \draw[line] (1.35,1.75) -- (1.35,2.25);
    
    \draw[line] (1.75,2.95) -- (2.25,2.95);
    \draw[line] (1.75,2.65) -- (2.25,2.65);
    
    \draw[line] (2.65,1.75) -- (2.65,2.25);
    \draw[line] (2.95,1.75) -- (2.95,2.25);
    
    \draw[line] (1.75,1.35) -- (2.25,1.35);
    \draw[line] (1.75,1.05) -- (2.25,1.05);
    
    % Slope
    \draw[dashed] (0,2) -- (4,2);
    
    \node[text=blue] at(0.5,3.4) {$\downarrow$};
    \node[text=blue] at(1.0,3.4) {$\downarrow$};
    \node[text=blue] at(1.5,3.4) {$\downarrow$};
    \node[text=blue] at(0.5,2.7) {$\downarrow$};
    \node[text=blue] at(1.0,2.7) {$\downarrow$};
    \node[text=blue] at(1.5,2.7) {$\downarrow$};
    
    \node[text=blue] at(2.45,3.4) {$\downarrow$};
    \node[text=blue] at(2.95,3.4) {$\downarrow$};
    \node[text=blue] at(3.45,3.4) {$\downarrow$};
    \node[text=blue] at(2.45,2.7) {$\downarrow$};
    \node[text=blue] at(2.95,2.7) {$\downarrow$};
    \node[text=blue] at(3.45,2.7) {$\downarrow$};
    
    \node[text=blue] at(1.975,2.8) {$\downarrow$};
    
    \node[text=blue] at(1.2,2.2) {$\downarrow$};
    \node[text=blue] at(2.8,2.2) {$\downarrow$};
\end{tikzpicture}
\qquad
\begin{tikzpicture}[scale=0.7]
    \draw (0,0) -- (4,0) -- (4,4) -- (0,4) -- cycle;
    \fill[yellow] (0.3,3.7) -- (0.8,3.7) -- (0.8,3.2) -- (0.3,3.2) -- cycle;
    % bottom-left
    \draw[line] (0.3,0.3) -- (0.3,1.75);
    \draw[line] (0.3,1.75) -- (1.05,1.75);
    \draw[line] (1.35,1.75) -- (1.75,1.75);
    \draw[line] (1.75,1.75) -- (1.75,1.35);
    \draw[line] (1.75,1.05) -- (1.75,0.3);
    \draw[line] (1.75,0.3) -- (0.3,0.3);
    
    % top-left
    \draw[line] (0.3,2.25) -- (0.3,3.7);
    \draw[line] (0.3,3.7) -- (1.75,3.7);
    \draw[line] (1.75,3.7) -- (1.75,2.95);
    \draw[line] (1.75,2.25) -- (1.75,2.65);
    \draw[line] (1.75,2.25) -- (1.35,2.25);
    \draw[line] (1.05,2.25) -- (0.3,2.25);
    
    % top-right
    \draw[line] (2.25,2.25) -- (2.25,2.65);
    \draw[line] (2.25,2.95) -- (2.25,3.7);
    \draw[line] (2.25,3.7) -- (3.7,3.7);
    \draw[line] (3.7,3.7) -- (3.7,2.25);
    \draw[line] (3.7,2.25) -- (2.95,2.25);
    \draw[line] (2.65,2.25) -- (2.25,2.25);
    
    % bottom-right
    \draw[line] (2.25,0.3) -- (2.25, 1.05);
    \draw[line] (2.25,1.35) -- (2.25, 1.75);
    \draw[line] (2.25,1.75) -- (2.65,1.75);
    \draw[line] (2.95,1.75) -- (3.7,1.75);
    \draw[line] (3.7,1.75) -- (3.7,0.3);
    \draw[line] (3.7,0.3) -- (2.25,0.3);
    
    % Hallways
    \draw[line] (1.05,1.75) -- (1.05,2.25);
    \draw[line] (1.35,1.75) -- (1.35,2.25);
    
    \draw[line] (1.75,2.95) -- (2.25,2.95);
    \draw[line] (1.75,2.65) -- (2.25,2.65);
    
    \draw[line] (2.65,1.75) -- (2.65,2.25);
    \draw[line] (2.95,1.75) -- (2.95,2.25);
    
    \draw[line] (1.75,1.35) -- (2.25,1.35);
    \draw[line] (1.75,1.05) -- (2.25,1.05);
    
    % Slope
    \draw[dashed] (0,2) -- (4,2);
    
    \node[text=red] at(0.5,3.4) {$\uparrow$};
    \node[text=red] at(1.0,3.4) {$\uparrow$};
    \node[text=red] at(1.5,3.4) {$\uparrow$};
    \node[text=red] at(0.5,2.7) {$\uparrow$};
    \node[text=red] at(1.0,2.7) {$\uparrow$};
    \node[text=red] at(1.5,2.7) {$\uparrow$};
    
    \node[text=red] at(2.45,3.4) {$\uparrow$};
    \node[text=red] at(2.95,3.4) {$\uparrow$};
    \node[text=red] at(3.45,3.4) {$\uparrow$};
    \node[text=red] at(2.45,2.7) {$\uparrow$};
    \node[text=red] at(2.95,2.7) {$\uparrow$};
    \node[text=red] at(3.45,2.7) {$\uparrow$};
    
    \node[text=red] at(1.975,2.8) {$\uparrow$};
    
    \node[text=red] at(1.2,2.2) {$\uparrow$};
    \node[text=red] at(2.8,2.2) {$\uparrow$};
\end{tikzpicture}
\caption{Illustration of the GWS (left) and the GWN (right) configurations of the \emph{GridWorld with Slope} setting. The arrows represent the slope, yellow boxes indicate the initial state distribution.}
\label{fig:gridslope_configs}
\end{figure}

==> submission/contents/figures/old/gridslope_entropy_comparison.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \includegraphics[scale=1]{contents/plot_files/img/gridslope_hist_ent_multi.pdf}
        \caption{Multiple}
        \label{fig:gridslope_hist_ent_multi}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \includegraphics[scale=1]{contents/plot_files/img/gridslope_hist_ent_north.pdf}
        \caption{GWN}
        \label{fig:gridslope_hist_ent_north}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.25\textwidth}
        \centering
        \includegraphics[scale=1]{contents/plot_files/img/gridslope_hist_ent_south.pdf}
        \caption{GWS}
        \label{fig:gridslope_hist_ent_south}
    \end{subfigure}
    \caption{Comparison between the optimal policies of each tested configuration: we plot the $\mathcal{E}_{\vcmp}^1(\pi)$ ($\alpha = 1$) obtained by running each optimal policy on GridWorld with both the environments sampled according to $p_{\vcmp} = [0.8,0.2]$ in \textbf{(a)}, on the \emph{adversarial} $GWN$ in \textbf{(b)} and on the \emph{easier} $GWS$ in \textbf{(c)}. The dashed line in \textbf{(b)} and \textbf{(c)} represents the optimal value of $\mathcal{E}_{\vcmp}^1(\pi)$ in that specific configuration. (95\% c.i. over 4 runs, $N_{traj} = 200$, $T = 400$).}
    \label{fig:gridslope_entropy_comparison}
\end{figure*}

==> submission/contents/figures/old/gridslope_entropy_dist_and_baseline.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{contents/plot_files/img/gridslope_ent_dist.pdf}
        \caption{$\mathcal{E}_{\vcmp}$}
        \label{fig:gridslope_entropy_distribution}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{contents/plot_files/img/gridslope_baseline.pdf}
        \caption{Baseline}
        \label{fig:gridslope_baselines_comparison}
    \end{subfigure}
    \caption{In \textbf{(a)} we show how the metric $\mathcal{E}_{\vcmp}$ is distributed, highlighting the loss of the \emph{double-tail} in MEMENTO ($p_{\vcmp} = [0.8, 0.2])$. In \textbf{(b)} we provide a comparison supporting the choice of our baseline $b = - \var (H_\tau)$. (95\% c.i. over 4 runs, $N_{traj} = 200$, $T = 400$).}
    \label{fig:gridslope_entropy_dist_and_baseline}
\end{figure*}

==> submission/contents/figures/old/gridslope_perc_dist.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.55\columnwidth]{contents/plot_files/img/gridslope_percentile_dist.pdf}
    \caption{Distribution of mini-batches inside the $\alpha$-percentile ($\alpha = 0.35$). We plot the number of batches that fall into the the $\alpha$-percentile for each configuration throughout the training. The two dotted lines represent the quantity that one could expect if considering the distribution $p_{\vcmp} = [0.8, 0.2]$ (95\% c.i. over 4 runs, $N_{traj} = 200$, $T = 400$).}
    \label{fig:gridslope_perc_dist}
\end{figure}

==> submission/contents/figures/old/gridslope_percentiles_comparison.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.9\columnwidth]{contents/plot_files/img/gridslope_percentiles_comparison.pdf}
    \caption{Comparison between optimal policies trained with different value of $\alpha$ (95\% c.i. over 4 runs, $N_{traj} = 200$, $T = 400$).}
    \label{fig:gridslope_percentiles_comparison}
\end{figure}

==> submission/contents/figures/old/multigrid_entropy_comparison.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{contents/plot_files/img/multigrid_entropy_estimation.pdf}
        \caption{Adversarial}
        \label{fig:multigrid_entropy_comparison_adv}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{contents/plot_files/img/multigrid_entropy_estimation_all_configs.pdf}
        \caption{Multiple}
        \label{fig:multigrid_entropy_comparison_multi}
    \end{subfigure}
    \caption{Comparison between MEMENTO and risk-neutral: we plot both $\mathcal{E}_{\vcmp}$ and $\mathcal{E}_{\vcmp}^{\alpha}$ with $\alpha = 0.1$ obtained by running the optimal policies on $\textbf{(a)}$ the \emph{adversarial} configuration and $\textbf{(b)}$ with all the 10 configurations, each one sampled with probability $p_{\cmp} = 0.1$. (95\% c.i. over 4 runs, $N_{traj} = 500$, $T = 400$).}
    \label{fig:multigrid_entropy_comparison}
\end{figure*}

==> submission/contents/figures/old/multigrid_goal_rl.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.85]{contents/plot_files/img/multigrid_goal_rl.pdf}
    \caption{Comparison of the average return as a function of learning epochs achieved by TRPO with MEMENTO initialization, TRPO with a risk-neutral policy as initialization and TRPO from scratch over a set of sparse-reward RL tasks in the adversarial configuration (95\% c.i. over 54 sampled goal locations).}
    \label{fig:multigrid_goal_rl}
\end{figure}

==> submission/contents/figures/problem.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.96\textwidth]{contents/images/problem.png}
    \caption{On the left, we highlight the unsupervised pre-training, in which the agent iteratively interacts with a CMP $\cmp \in \vcmp$ drawn from $p_\cmp$. The pre-trained policy $\pi^*_{\mathcal{E}}$ conveys the initialization to the subsequent supervised fine-tuning (on the right), which outputs a reward maximizing policy $\pi_{\mathcal{J}}^*$ for an MDP $\cmp \cup R$ that pairs $\cmp \in \vcmp$ with an arbitrary reward function $R$.}
    \label{fig:problem}
    %\vspace{-0.3cm}
\end{figure*}

==> submission/contents/figures/related_work.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{contents/images/related_work.png}
    \caption{Where our work (star) stands in the literature.}
    \label{fig:related_work}
\end{figure}

==> submission/contents/sections/conclusions.tex <==
% In this paper, we addressed the problem of learning to explore a class of multiple reward-free environments with a unique general strategy. First, we cast the problem into the familiar MSVE framework, where we considered the maximization of a critical percentile of the state visitation entropy. Then, we presented MEMENTO, a policy gradient algorithm to optimize the exploration objective via mediated interactions with the class of environments. Finally, we provided an extensive experimental analysis to show the ability of MEMENTO in learning to explore challenging classes of continuous environments and to highlight the benefit that the resulting exploration strategy brings to RL problems specified over the same classes.
In this paper, we addressed the problem of learning to explore a class of multiple reward-free environments with a unique general strategy. First, we formulated the problem within a tractable MSVE objective with percentile sensitivity. Then, we presented a policy gradient algorithm to optimize this objective. Finally, we provided an extensive experimental analysis to show its ability in learning to explore and the benefits it brings to subsequent RL problems.
We believe that this paper motivates the importance of designing specific solutions to the relevant reward-free exploration problem over multiple environments.

%As a final note, it is worth mentioning an alternative problem formulation in which MEMENTO can be employed with benefit. 
%Especially, we could replace the class of environments of our setting with a single CMP specified under uncertainty~\citep{satia1973markovian}, and deal with the \emph{robust reward-free exploration} problem with little or no modifications to MEMENTO.
% On an orthogonal line, one could pursue reward-free exploration of a class of multiple \emph{vision-based domains}. In this case, MEMENTO could be employed in combination with a proper metric learned over images, as proposed in~\citep{anonymous2021unsupervised} for an environment-specific setting.


==> submission/contents/sections/experiments.tex <==
In this section, we provide an extensive empirical evaluation of the proposed methodology over the two-phase learning process described in Figure~\ref{fig:problem}, which is organized as follows:
\begin{itemize} \compresslist
    \item[\ref{sec:experiments_learning_to_explore_illlustrative}]
    We show the ability of our method in learning to explore a class of illustrative continuous gridworlds, emphasizing the importance of the percentile sensitivity;
    \item[\ref{sec:experiments_alpha_sensitivity}]
    We discuss how the choice of the percentile of interest affects the exploration strategy;
    \item[\ref{sec:experiments_rl_illustrative}]
    We highlight the benefit that the exploration strategy provides to RL on the same class;
    \item[\ref{sec:experiments_scalability_class}]
    We verify the ability of our method to scale with the size of the class of environments, by considering a class of 10 continuous gridworlds;
    \item[\ref{sec:experiments_scalability_dimension}]
    We verify the ability of our method to scale with the dimensionality of the environments in the class, by considering a class of 29D continuous control Ant domains;
    \item[\ref{sec:experiments_scalability_vision}] We verify the ability of our method to scale with visual inputs, by considering a class of 147D MiniGrid~\citep{chevalier2018minimalistic} domains;
    \item[\ref{sec:experiments_meta}]
    We show that the exploration strategy learned with our approach is superior for RL \wrt a policy meta-trained with MAML~\citep{finn2017model, gupta2018unsupervised} on the same class.
\end{itemize}
A thorough description of the experimental setting is provided in Appendix~\ref{apx:experiments}.

\input{contents/figures/gridslope}
\subsection{Learning to Explore Multiple Environments with Percentile Sensitivity}
\label{sec:experiments_learning_to_explore_illlustrative}
In this section, we consider a class $\vcmp$ composed of two different configurations of a continuous gridworld domain with 2D states and 2D actions, which we call the \emph{GridWorld with Slope}. In each configuration, the agent navigates through four rooms connected by narrow hallways, by choosing a (bounded) increment along the coordinate directions. A visual representation of the setting can be found in Figure~\ref{fig:gridslope_illustration}, where the shaded areas denote the initial state distribution and the arrows render a slope that favors or contrasts the agent's movement. The configuration on the left has a south-facing slope, and thus it is called GridWorld with South slope (GWS). Instead, the one on the right is called GridWorld with North slope (GWN) as it has a north-facing slope. This class of environments is unbalanced (and thus interesting to our purpose) for two reasons: First, the GWN configuration is more challenging from a pure exploration standpoint, since the slope prevents the agent from easily reaching the two bottom rooms; secondly, the distribution over the class is also unbalanced, as it is $p_{\vcmp} = [Pr(\text{GWS}), Pr(\text{GWN})] = [0.8, 0.2]$.
In this setting, we compare  MEMENTO against \emph{Neutral}, which is a simplified version of MEMENTO with $\alpha = 1$,\footnote{The pseudocode is identical to Algorithm~\ref{alg:memento} except that all trajectories affect the gradient estimate in~\eqref{eq:policy_gradient_estimator}.} to highlight the importance of percentile sensitivity \wrt a na\"ive approach to the multiple environments scenario. The methods are evaluated in terms of the state visitation entropy $\mathcal{E}_{\vcmp}^1$ induced by the exploration strategies they learn.

In Figure~\ref{fig:gridslope_exploration}, we compare the performance of the optimal exploration strategy obtained by running MEMENTO ($\alpha=0.2$) and Neutral ($\alpha=1$) for 150 epochs on the GridWorld with Slope class ($p_{\vcmp} = [0.8, 0.2]$). We show that the two methods achieve a very similar expected performance over the class (Figure~\ref{fig:gridslope_exploration_all}). However, this expected performance is the result of a (weighted) average of very different contributions. As anticipated, Neutral has a strong performance in GWS ($p_{\vcmp} = [1, 0]$, Figure~\ref{fig:gridslope_exploration_south}), which is close to the configuration-specific optimum (dashed line), but it displays a bad showing in the adverse GWN ($p_{\vcmp} = [0, 1]$, Figure~\ref{fig:gridslope_exploration_north}). Conversely, MEMENTO learns a strategy that is much more robust to the configuration, showing a similar performance in GWS and GWN, as the percentile sensitivity prioritizes the worst case during training. 
To confirm this conclusion, we look at the actual distribution that is generating the expected performance in Figure~\ref{fig:gridslope_exploration_all}. In Figure~\ref{fig:gridslope_empirical_distribution}, we provide the empirical distribution of the trajectory-wise performance ($H_\tau$), considering a batch of 200 trajectories with $p_{\vcmp} = [0.8, 0.2]$. It clearly shows that Neutral is heavy-tailed towards lower outcomes, whereas MEMENTO concentrates around the mean. \emph{This suggests that with a conservative choice of $\alpha$ we can induce a good exploration outcome for every trajectory (and any configuration), while without percentile sensitivity we cannot hedge against the risk of particularly bad outcomes.} However, let us point out that not all classes of environments would expose such an issue for a na\"ive, risk-neutral approach (see Appendix~\ref{apx:counterexample} for a counterexample), but it is fair to assume that this would arguably generalize to any setting where there is an imbalance (either in the hardness of the configurations, or in their sampling probability) in the class. These are the settings we care about, as they require nuanced solutions (\eg MEMENTO) for scenarios with multiple environments.
\input{contents/figures/gridslope_rl}

% we provide a comparison directed at showing empirically the claim presented in Section 4. We show that the CVaR optimization as in (\ref{eq:exp_risk_averse}), combined to the sampling procedure in $\vcmp$, leads to a more robust exploratory policy, i.e. able to generalize through different environments, without suffering a drop in performance due to some adversarial configurations.
% We carry out the evaluation on a custom version of GridWorld (2D states, 2D actions), which we coded from scratch. An illustration to facilitate the comprehension of the setting is shown in Figure \ref{fig:gridslope_illustration}. The agent can move inside a map composed of four rooms connected by four hallways, by choosing at each step how much to move on the x and y axes. There are two configurations sharing this spatial context, each one characterized by a different level of complexity: we denote the \emph{easy} one as $GWS$ (GridWorld with South slope), since it is characterized by a south-facing slope, while $GWN$ (GridWorld with North slope) is the \emph{adversarial} one and it is characterized by a north-facing slope. Both the slopes are applied only in the upper half of the environment. Because of the way in which the initial position of the agent is determined, $GWN$ has a higher level of complexity, since at least in the first epochs the agent will continuously collide with the top-border of the environment, leading in general to a much more lower entropy \wrt to $GWS$. The two environments $GWS$ and $GWN$ are drawn according to a specified non-uniform distribution $p_{\vcmp} = [0.8, 0.2]$, meaning that the \emph{adversarial} configuration is sampled only with a probability of $0.2$, as a representative of the \emph{worst-case} scenario.
% In Figure \ref{fig:gridslope_exploration} we depict a comparison showing the performance of the optimal policy in each configuration. From Figure \ref{fig:gridslope_exploration_all} one can see that MEMENTO is able to obtain an exploration comparable to the one of the risk-neutral approach in the \emph{multi-environment} scenario. Figure \ref{fig:gridslope_exploration_north} considers the \emph{adversarial} configuration $GWN$ ($p_{\vcmp} = [0, 1]$) and it demonstrates that our approach outclasses the risk-neutral one, which instead obtains a performance comparable to the policy trained with only south-facing slope. Finally, Figure \ref{fig:gridslope_exploration_south} illustrates how our approach, although performing worse than the risk-neutral one, still results in a good exploration also in $GWS$ ($p_{\vcmp} = [1, 0]$): crucially, the gap here is definitely smaller than the gap in Figure \ref{fig:gridslope_exploration_north}. Overall, it is clear that MEMENTO manages to learn a policy which is is able to crosswise explore $\vcmp$, without suffering the presence of a challenging configuration. In order to corroborate such result, in Figure \ref{fig:gridslope_empirical_distribution} we give a visualization of the way in which the metric $\mathcal{E}_{\vcmp}$ is distributed, plotting the number of mini-batches that fall in a specific range of values. Crucially, the \emph{double-tail} behaviour of the risk-neutral policy disappears with MEMENTO, meaning the \emph{elimination of the risk} in exchange for a small lowering of the average performance. In Figure \ref{fig:gridslope_alpha_composition} we instead show the proportion according to which the mini-batches fall in the $\alpha$-percentile. Clearly, the percentage of mini-batches containing trajectories sampled from the \emph{adversarial} configuration $GWN$ is always above the threshold drawn according to the distribution $p_{\vcmp} = [0.8, 0.2]$, reaching the cap of almost 60\% ($\sim$ 8 mini-batches) towards the end. Additionally, in Figure \ref{fig:gridslope_baselines_comparison} we empirically motivate the choice of the convenient baseline $b = - \var (H_\tau)$. No advantage derives from the use of the $\var$ baseline; in fact, it leads to a slightly higher variance, as depicted in the right plot, with the mean of the gradients of the last layer of the policy, i.e. the \emph{mean actions} $\bm{\mu}_{\vtheta}(\bm{s})$ one.

\subsection{On the Value of the Percentile}
\label{sec:experiments_alpha_sensitivity}
In this section, we consider repeatedly training MEMENTO with different values of $\alpha$ in the GridWorld with Slope domain, and we compare the resulting exploration performance $\mathcal{E}_{\vcmp}^1$ as before. In Figure~\ref{fig:gridslope_alpha}, we can see that the lower $\alpha$ we choose, the more we prioritize GWN (right bar for every $\alpha$) at the expense of GWS (left bar). Note that this trend carries on with increasing $\alpha$, ending in the values of Figures~\ref{fig:gridslope_exploration_south},~\ref{fig:gridslope_exploration_north}. The reason for this behavior is quite straightforward, the smaller is $\alpha$, the larger is the share of trajectories from the adverse configuration (GWN) ending up in the percentile at first, and thus the more GWN affects the policy update (see the gradient in~\eqref{eq:policy_gradient_estimator}). 
\emph{Note that the value of the percentile $\alpha$ should not be intended as a hyper-parameter to tune via trial and error, but rather as a parameter to select the desired risk profile of the algorithm.}
Indeed, there is not a way to say which of the outcomes in Figure~\ref{fig:gridslope_alpha} is preferable, as they are all reasonable trade-offs between the average and worst-case performance, which might be suited for specific applications.
For the sake of consistency, in every experiment of our analysis we report results with a value of $\alpha$ that matches the sampling probability of the worst-case configuration, but similar arguments could be made for different choices of $\alpha$.
% One might ask how much the dimension of the percentile $\alpha$ affects the results. In Figure \ref{fig:gridslope_alpha} we report a comparison on both the configurations $GWN$ and $GWS$. The trade-off is plainly visible: a higher $\alpha$ positively impacts the exploration in $GWS$, due to the presence of more mini-batches with its own trajectories, with the drawback of a worse performance on the \emph{adversarial} $GWN$, and vice-versa. 

\subsection{RL with a General Exploration Strategy}
\label{sec:experiments_rl_illustrative}
%In this section, we illustrate how beneficial is the pre-trained exploration strategy to deal with any RL problem one could specify in the GridWorld with Slope class.
To assess the benefit of the pre-trained strategy, we design a family of MDPs $\cmp^R$, where $\cmp \in \{\text{GWS},\text{GWN}\}$, and $R$ is any sparse reward function that gives 1 when the agent reaches the area nearby a random goal location and 0 otherwise. On this family, we compare the performance achieved by TRPO~\citep{schulman2015trust} with different initializations: The exploration strategies learned (as in Section~\ref{sec:experiments_learning_to_explore_illlustrative}) by MEMENTO ($\alpha = 0.2$) and Neutral ($\alpha=1$), or a randomly initialized policy (Random). These three variations are evaluated in terms of their average return $\mathcal{J}_{\cmp^R}$, which is defined in~\eqref{eq:rl_objective}, over 50 randomly generated goal locations (Figure~\ref{fig:gridslope_sampled_goals}).
As expected, the performance of TRPO with Neutral is competitive in the GWS configuration (Figure~\ref{fig:gridslope_rl}), but it falls sharply in the GWN configuration, where it is not significantly better than TRPO with Random. Instead, the performance of TRPO with MEMENTO is strong on both GWS and GWN. Despite the simplicity of the domain, solving an RL problem in GWN with an adverse goal location is far-fetched for both a random initialization and a na\"ive solution to the reward-free exploration over multiple environments.
% We now illustrate how a learning agent can benefit from an exploration policy learned by MEMENTO in a sparse-reward RL setting, defined over the same class of environments. Especially, we compare the performance achieved by TRPO \cite{schulman2015trust} initialized with a MEMENTO policy \wrt TRPO initialized with a \emph{risk-neutral} policy and TRPO starting from scratch, i.e. with a randomly initialized policy. We consider the two configurations $GWS$ and $GWN$ and for each of them we make an evaluation in terms of average return on a series of sparse-reward RL tasks. In particular, we run 54 experiments, each one with a different randomly sampled goal location (see Figure \ref{fig:gridslope_sampled_goals}): the reward is 1 in the states having Euclidean distance to the goal lower than 0.1, while it is zero in all the remaining state space. As we show in Figure \ref{fig:gridslope_rl}, the MEMENTO initialization leads to a drastically better result in the \emph{adversarial} configuration $GWN$, while retaining a good performance in $GWS$. Notably, the \emph{risk-neutral} approach in $GWN$ is even comparable with the random initialization, probably because highly biased towards the south-slope configuration.

\input{contents/figures/multigrid_ant}
\subsection{Scaling to Larger Classes of Environments}
\label{sec:experiments_scalability_class}
In this section, we consider a class $\vcmp$ composed of ten different configurations of the continuous gridworlds presented in Section~\ref{sec:experiments_learning_to_explore_illlustrative} (including the GWN as the worst-case configuration) which we call the \emph{MultiGrid} domain. As before, we compare MEMENTO ($\alpha = 0.1$) and Neutral ($\alpha=1$) on the exploration performance $\mathcal{E}_{\vcmp}^{1}$ achieved by the optimal strategy, in this case considering a uniformly distributed $p_{\vcmp}$. While the average performance of Neutral is slightly higher across the class (Figure~\ref{fig:multigrid} left, left bar), MEMENTO still has a decisive advantage in the worst-case configuration (Figure~\ref{fig:multigrid} left, right bar). Just as in Section~\ref{sec:experiments_rl_illustrative}, this advantage transfer to RL, where we compare the average return $\mathcal{J}_{\cmp^R}$ achieved by TRPO with MEMENTO, Neutral, and Random initializations over 50 random goal locations in the GWN configuration (Figure~\ref{fig:multigrid} right). \emph{Whereas in the following sections we will only consider classes of two environments, this experiment shows that the arguments made for small classes of environments can easily generalize to larger classes.}
% In this section, we extend the previous analysis by assessing the capability of MEMENTO to scale to a larger number of environments. Especially, we consider a set of 10 GridWorld environments. The \emph{adversarial} configuration is the same as in Section \ref{subsec:risk_averse}, i.e. $GWN$, while the remaining 9 environments are characterized by different slopes (towards south, east, south-east) or by no slope at all, so that their exploration is not completely straightforward, but still easier than the adversarial one.
% Also in this case, in Figure \ref{fig:multigrid} we show the performance of MEMENTO compared to the risk-neutral approach. More precisely, the comparison is made in the \emph{adversarial configuration} (Figure \ref{fig:multigrid_exploration_worst}) and in the \emph{multiple configurations} scenario (Figure \ref{fig:multigrid_exploration_all}). In this last case, each environment is sampled with $p_{\cmp} = 0.1$. Although the difference is not as conspicuous as in the \emph{2-environments} experiment, MEMENTO still has a decisive advantage in terms of exploration in the difficult setting, while retaining an optimal performance in the multi-environment one.
% We report in Figure~\ref{fig:multigrid_rl} the RL analysis, carried out as in Section \ref{subsec:risk_averse}. We considered the same goal locations of Figure~\ref{fig:gridslope_sampled_goals}, randomly sampled in the \emph{adversarial} configuration. Even with 10 environments, different in geometrical structure and type of slope, the MEMENTO initialization leads to better performance.

\subsection{Scaling to Increasing Dimensions}
\label{sec:experiments_scalability_dimension}
In this section, we consider a class $\vcmp$ consisting of two Ant environments, with 29D states and 8D actions. In the first, sampled with probability $p_{\cmp_1} = 0.8$, the Ant faces a wide descending staircase (\emph{Ant Stairs Down}). In the second, the Ant faces a narrow ascending staircase (\emph{Ant Stairs Up}, sampled with probability $p_{\cmp_2} = 0.2$), which is significantly harder to explore than the former. In the mold of the gridworlds in Section~\ref{sec:experiments_learning_to_explore_illlustrative}, these two configurations are specifically designed to create an imbalance in the class. As in Section~\ref{sec:experiments_learning_to_explore_illlustrative}, we compare MEMENTO ($\alpha = 0.2$) against Neutral ($\alpha = 1$) on the exploration performance $\mathcal{E}_{\vcmp}^{1}$ achieved after 500 epochs. MEMENTO fares slightly better than Neutral both in the worst-case configuration (Figure~\ref{fig:ant} left, right bar) and, surprisingly, in the easier one (Figure~\ref{fig:ant} left, left bar).\footnote{Note that this would not happen in general, as we expect MEMENTO to be better in the worst-case but worse on average. Apparently, the percentile objective positively biases the average performance in this setting.}
Then, we design a set of incrementally challenging sparse-rewards RL tasks in the \emph{Ant Stairs Up}, which give reward 1 upon reaching a certain step of the staircase. Also in this setting, TRPO with Memento initialization outperforms TRPO with Neutral and Random in terms of the average return $\mathcal{J}_{\cmp^R}$ (Figure~\ref{fig:ant} right). Note that these sparse-reward continuous control tasks are particularly arduous: TRPO with Neutral and Random barely learns anything, while even TRPO with MEMENTO does not handily reach the optimal average return (1). %especially in the tasks associated to the upper steps of the staircase.

\input{contents/figures/meta}
\subsection{Scaling to Visual Inputs}
\label{sec:experiments_scalability_vision}
In this section, we consider a class $\vcmp$ of two partially-observable MiniGrid~\citep{chevalier2018minimalistic} environments, in which the observation is a 147D image of the agent's field of view. 
In Figure~\ref{fig:minigrid_visualization}, we provide a visualization of the domain: The easier configuration (EasyG, left) is sampled with probability $p_{\cmp_1} = 0.8$, the adverse configuration (AdvG, right) is sampled with probability $p_{\cmp_2} = 0.2$. Two factors make the AdvG more challenging to explore, which are the presence of a door at the top-left of the grid, and reversing the effect of agent's movements (\eg the agent goes backward when it tries to go forward). 
Whereas in all the previous experiments we estimated the entropy on the raw input features, visual inputs require a wiser choice of a metric. As proposed in~\citep{seo2021state}, we process the observations through a random encoder before computing the entropy estimate in~\eqref{eq:knn_entropy_estimator}, while keeping everything else as in Algorithm~\ref{alg:memento}. We run this slightly modified version of MEMENTO ($\alpha = 0.2$) and Neutral ($\alpha = 1$) for 300 epochs. Then, we compare TRPO with the learned initializations (as well as Random) on sparse-reward tasks defined upon the class. As in previous settings, TRPO with MEMENTO results slightly worse than TRPO with Neutral in the easier configuration (Figure~\ref{fig:minigrid}, left), but significantly better in the worst-case (Figure~\ref{fig:minigrid}, right). Notably, TRPO from scratch struggles to learn the tasks, especially in the AdvG (Figure~\ref{fig:minigrid}, right).
\emph{Although the MiniGrid domain is extremely simple from a vision standpoint, we note that the same architecture can be employed in more challenging scenarios~\citep{seo2021state}, while the focus of this experiment is the combination between visual inputs and multiple environments.}

\subsection{Comparison with Meta-RL}
\label{sec:experiments_meta}
In this section, we compare our approach against meta-training a policy with MAML~\citep{finn2017model} on the same \emph{GridWorld with Slope} ($p_{\vcmp} = [0.8, 0.2]$) and \emph{MultiGrid} (uniformly distributed $p_{\vcmp}$) domains that we have previously presented. 
Especially, we consider two relevant baselines. The first is MAML+R, to which we provide full access to the tasks (\ie rewards) during meta-training. Note that this gives MAML+R an edge over MEMENTO, which operates reward-free training. The second is MAML+DIAYN~\citep{gupta2018unsupervised}, which operates unsupervised meta-training through an intrinsic reward function learned with DIAYN~\citep{eysenbach2018diversity}.
As in previous sections, we consider the average return $\mathcal{J}_{\cmp^R}$ achieved by TRPO initialized with the exploration strategy learned by MEMENTO or the meta-policy learned by MAML+R and MAML+DIAYN. TRPO with MEMENTO fares clearly better than TRPO with the meta-policies in all the configurations (Figures~\ref{fig:maml_gridslope}, \ref{fig:maml_multigrid}). Even if it works fine in fast adaptation (see Appendix~\ref{apx:meta_experiments_details}), \emph{MAML struggles to encode the diversity of task distribution into a single meta-policy and to deal with the most adverse tasks in the long run.} Moreover, DIAYN does not specifically handle multiple environments, and it fails to cope with the larger \emph{MultiGrid} class.
%(see Appendix~\ref{apx:meta_experiments_details}).

==> submission/contents/sections/introduction.tex <==
% RL limitation
The typical Reinforcement Learning~\citep[RL,][]{sutton2018reinforcement} setting involves a learning agent interacting with an environment in order to maximize a reward signal. In principle, the reward signal is a given and perfectly encodes the task. In practice, the reward is usually hand-crafted, and designing it to make the agent learn a desirable behavior is often a huge challenge. This poses a serious roadblock on the way of autonomous learning, as any task requires a costly and specific formulation, while the synergy between solving one RL problem and another is very limited.
% Reward-free RL
To address this crucial limitation, \citet{jin2020rewardfree} have formulated the \emph{reward-free} RL problem. In this setting, the agent is tasked with mastering an environment without rewards, so that the knowledge it acquires can be eventually deployed to solve any RL problem one could specify in this same environment. \emph{Mastering} the environment has been formulated in (i) \emph{learning to model} its transition dynamics up to a convenient confidence \citep{jin2020rewardfree,tarbouriech2020active}, or (ii) \emph{learning to explore} it with a general, task-agnostic, strategy~\citep{hazan2019maxent}. Although they overcome the reliance on a reward function, all of the previous solutions to reward-free RL are still severely environment-specific.

% General problem
In this work, we aim to push the generality of reward-free learning even further by addressing the problem of \emph{learning to explore multiple environments} with a single exploration strategy. In this setting, the agent faces a class of reward-free environments that belong to the same domain but differ in their transition dynamics. At each turn of the learning process, the agent is drawn into an environment within the class, where it can interact for a finite number of steps before facing another turn. The process carries on sequentially for a finite number of turns. The ultimate goal of the agent is to learn an exploration strategy that helps to solve any subsequent RL task specified over the class.
%reducing the burden on manual reward design while improving learning efficiency over RL from scratch.

% Our contributions
Our contribution to the problem is three-fold: (c1) We frame it into a tractable \emph{formulation} (Section~\ref{sec:problem}), (c2) we propose a \emph{methodology} to address it (Section~\ref{sec:method}), for which (c3) we provide a thorough \emph{empirical} evaluation (Section~\ref{sec:experiments}).
First, we extend a reward-free objective meant for environment-specific exploration, which is the \emph{Maximum State Visitation Entropy}~\citep[MSVE,][]{hazan2019maxent}. The underlying intuition is that a general exploration strategy has to visit with high probability any state where the agent might be rewarded in a subsequent RL task. When dealing with multiple environments, this becomes a \emph{multi-objective} problem, as one could establish any combination of preferences over the environments. In this work, instead of na\"ively optimizing the mean of the state visitation entropy across the class, we consider its Conditional Value-at-Risk~\citep[CVaR,][]{rockafellar2000optimization} to prioritize performance in particularly rare or adverse environments. 
We propose a policy gradient algorithm~\citep{deisenroth2013survey}, \emph{Multiple Environments Maximum ENTropy Optimization} (MEMENTO), to optimize the learning objective via mere interactions with the class of environments. As in recent works~\citep{mutti2020policy,anonymous2021unsupervised,seo2021state}, the algorithm employs non-parametric methods to deal with state entropy estimation in continuous and high-dimensional environments. Then, it leverages these estimated values to optimize the CVaR of the entropy by following its policy gradient~\citep{tamar2015optimizing}.
Finally, we provide an experimental analysis of the proposed method in a two-stage setting. First, we show that it is effective in training general exploration strategies over classes of continuous and high-dimensional environments without rewards. Second, we test the obtained exploration strategies as initialization for a number of RL tasks defined over the same class. Notably, the trained exploration strategy allows us to solve sparse-rewards tasks that are impractical to learn from scratch, while being robust to the most unfavorable environment thanks to the CVaR objective.
Related works are in Section~\ref{sec:related_work}, a preliminary theoretical analysis is in Appendix~\ref{sec:theory}, the proofs of the theorems are in Appendix~\ref{apx:proofs}. 
%The implementation of MEMENTO can be found at \url{https://github.com/muttimirco/memento}.


==> submission/contents/sections/method.tex <==
In this section, we present an algorithm, called \emph{Multiple Environments Maximum ENTropy Optimization} (MEMENTO), to optimize the exploration objective in~\eqref{eq:exp_risk_averse}
through mediated interactions with a class of continuous environments. 

MEMENTO operates as a typical policy gradient approach \citep{deisenroth2013survey}. It directly searches for an optimal policy by navigating a set of parametric differentiable policies $\Pi_{\Theta} := \lbrace \pi_{\vtheta} : \vtheta \in \Theta \subseteq \reals^n \rbrace$. It does so by repeatedly updating the policy parameters $\vtheta$ in the gradient direction, until a stationary point is reached. This update has the form
\begin{equation*}
    \vtheta ' = \vtheta + \beta \nabla_{\vtheta} \mathcal{E}_{\vcmp}^{\alpha} (\pi_{\vtheta}),
\end{equation*}
where $\beta$ is a learning rate, and $\nabla_{\vtheta} \mathcal{E}_{\vcmp}^{\alpha} (\pi_{\vtheta})$ is the gradient of~\eqref{eq:exp_risk_averse} \wrt $\vtheta$. The following proposition provides the formula of $\nabla_{\vtheta} \mathcal{E}_{\vcmp}^{\alpha} (\pi_{\vtheta})$. The derivation follows closely the one in~\citep[][Proposition 1]{tamar2015optimizing}, which we have adapted to our objective function of interest~\eqref{eq:exp_risk_averse}.
\begin{restatable}[]{prop}{cvarPolicyGradient}
The policy gradient of the exploration objective $\mathcal{E}_{\vcmp}^{\alpha} (\pi_{\vtheta})$ \wrt $\vtheta$ is given by
\begin{align}
    \nabla_{\vtheta} & \mathcal{E}_{\vcmp}^{\alpha} (\pi_{\vtheta}) =
    \EV_{\substack{\cmp \sim p_{\vcmp} \\ \tau \sim p_{\pi_{\vtheta},\cmp}}} 
    \bigg[ \bigg( \sum_{t = 0}^{T - 1} \nabla_{\vtheta} \log \pi_{\vtheta} (a_{t,\tau}|s_{t,\tau}) \bigg) \nonumber \\
    &\times \bigg( H_{\tau} - \var (H_\tau) \bigg) \bigg| H_{\tau} \leq \var (H_\tau) \bigg].
\end{align}
\label{prop:cvar_policy_gradient}
\end{restatable}
However, in this work we do not assume full knowledge of the class of CMPs $\vcmp$, and the expected value in Proposition~\ref{prop:cvar_policy_gradient} cannot be computed without having access to $p_{\vcmp}$ and $p_{\pi_{\vtheta}, \cmp}$. Instead, MEMENTO computes the policy update via a Monte Carlo estimation of $\nabla_{\vtheta} \mathcal{E}_{\vcmp}^{\alpha}$ from the sampled interactions $\lbrace (\cmp_i, \tau_i) \rbrace_{i = 1}^N$ with the class of environments $\vcmp$. The policy gradient estimate itself relies on a Monte Carlo estimate of each entropy value $H_{\tau_i}$ from $\tau_i$, and a Monte Carlo estimate of $\var (H_\tau)$ given the estimated $\lbrace H_{\tau_i} \rbrace_{i = 1}^N$. The following paragraphs describe how these estimates are carried out, while Algorithm~\ref{alg:memento} provides the pseudocode of MEMENTO. Additional details and implementation choices can be found in Appendix~\ref{apx:algorithm}.
\begin{algorithm}[t]
\caption{MEMENTO}
\label{alg:memento}
    \textbf{Input}: percentile $\alpha$, learning rate $\beta$\\
    \textbf{Output}: policy $\pi_{\bm{\theta}}$
    \begin{algorithmic}[1] %[1] enables line numbers
        \STATE initialize $\vtheta$
        \FOR{epoch $= 0,1,\ldots$, until convergence}
        \FOR{$i = 1,2,\ldots, N$}
        \STATE{sample an environment $\mathcal{M}_i \sim p_{\vcmp}$}
        \STATE sample a trajectory $\tau_i \sim p_{\pi_{\vtheta}, \cmp_i}$
        \STATE estimate $H_{\tau_i}$ with~\eqref{eq:knn_entropy_estimator}
        \ENDFOR
        \STATE estimate $\var (H_\tau)$ with~\eqref{eq:var_estimator}
        \STATE estimate $\nabla_{\vtheta} \mathcal{E}_{\vcmp}^{\alpha} (\pi_{\vtheta})$ with~\eqref{eq:policy_gradient_estimator}
        \STATE update parameters $\vtheta \gets \vtheta + \beta \widehat{\nabla}_{\vtheta} \mathcal{E}_{\cmp}^{\alpha} (\pi_{\vtheta})$
        \ENDFOR
    \end{algorithmic}
\end{algorithm}

\paragraph{Entropy Estimation}
We would like to compute the entropy $H_{\tau_i}$ of the state visitation frequencies $d_{\tau_i}$ from a single realization $\lbrace s_{t,\tau_i} \rbrace_{t=0}^{T - 1} \subset \tau_i$. This estimation is notoriously challenging when the state space is continuous and high-dimensional $\sspace \subseteq \reals^p$. Taking inspiration from recent works pursuing the MSVE objective~\citep{mutti2020policy,anonymous2021unsupervised,seo2021state}, we employ a principled $k$-Nearest Neighbors ($k$-NN) entropy estimator~\citep{singh2003nearest} of the form
\begin{equation}
    \widehat{H}_{\tau_i} \propto - \frac{1}{T} \sum_{t = 0}^{T - 1}
    \log \frac{k \ \Gamma (\frac{p}{2} + 1)}{T \ \big\| s_{t,\tau_i} - s^{k\text{-NN}}_{t, \tau_i} \big\|^p \ \pi^{\frac{p}{2}}},
    \label{eq:knn_entropy_estimator}
\end{equation}
where $\Gamma$ is the Gamma function, $\|\cdot\|$ is the Euclidean distance, and $s_{t, \tau_i}^{k\text{-NN}} \in \tau_i$ is the $k$-nearest neighbor of $s_{t,\tau_i}$. The intuition behind the estimator in $\eqref{eq:knn_entropy_estimator}$ is straightforward: We can suppose the state visitation frequencies $d_{\tau_i}$ to have a high entropy as long as the average distance between any encountered state and its $k$-NN is large. Despite its simplicity, a Euclidean metric suffices to get reliable entropy estimates in continuous control domains~\citep{mutti2020policy}.

\paragraph{VaR Estimation and Baseline}
The last missing piece to get a Monte Carlo estimate of the policy gradient $\nabla_{\vtheta} \mathcal{E}_{\vcmp}^\alpha$ is the value of $\var (H_\tau)$. Being $H_{[1]}, \ldots, H_{[N]}$ the order statistics out of the estimated values $\lbrace \widehat{H}_{\tau_i} \rbrace_{i = 1}^N$, we can na\"ively estimate the VaR as
\begin{equation}
    \evar (H_\tau) = H_{[\lceil \alpha N \rceil]}.
    \label{eq:var_estimator}
\end{equation}
Albeit asymptotically unbiased, the VaR estimator in~\eqref{eq:var_estimator} is known to suffer from a large variance in finite sample regimes~\citep{kolla2019concentration}, which is aggravated by the error in the upstream entropy estimates, which provide the order statistics.
This variance is mostly harmless when we use the estimate to filter out entropy values beyond the $\alpha$\%, \ie the condition $H_\tau \leq \var (H_\tau)$ in Proposition~\ref{prop:cvar_policy_gradient}. Instead, its impact is significant when we subtract it from the values within the $\alpha$\%, \ie the term $H_\tau - \var (H_\tau)$ in Proposition~\ref{prop:cvar_policy_gradient}. 
To mitigate this issue, we consider a convenient baseline $b = - \var (H_\tau)$ to be subtracted from the latter, which gives the Monte Carlo policy gradient estimator
\begin{equation}
    \widehat{\nabla}_{\vtheta} \mathcal{E}_{\vcmp}^\alpha (\pi_{\vtheta})
    = \sum_{i = 1}^N  f_{\tau_i} \ \widehat{H}_{\tau_i} \ \ind (\widehat{H}_{\tau_i} \leq \evar (H_\tau)),
    \label{eq:policy_gradient_estimator}
\end{equation}
where $f_{\tau_i} = \sum_{t = 0}^{T - 1} \nabla_{\vtheta} \log \pi_{\vtheta} (a_{t,\tau_i}|s_{t,\tau_i})$. Notably, the baseline $b$ trades off a lower estimation error for a slight additional bias in the estimation~\eqref{eq:policy_gradient_estimator}. We found that this baseline leads to empirically good results and we provide some theoretical corroboration over its benefits in Appendix~\ref{apx:algorithm_baseline}.


==> submission/contents/sections/preliminaries.tex <==
In this section, we report background and notation. A vector $\bm{v}$ is denoted in bold, and $v_i$ stands for its $i$-th entry.

\paragraph{Probability and Percentiles}
Let $X$ be a random variable distributed according to a cumulative density function (cdf) $F_X (x) = Pr (X \leq x)$. We denote with $\EV [X]$, $\Var [X]$ the expected value and the variance of $X$ respectively.
Let $\alpha \in (0, 1)$ be a confidence level, we call the $\alpha$-percentile (shortened to $\alpha$\%) of the variable $X$ its Value-at-Risk (VaR), which is defined as
$$
    \var (X) = \inf \big\lbrace x \;|\; F_X (x) \geq \alpha \big\rbrace.
$$
Analogously, we call the mean of this same $\alpha$-percentile the Conditional Value-at-Risk (CVaR) of $X$,
$$
    \cvar (X) = \EV \big[ X \;|\; X \leq \var (X) \big].
$$

\paragraph{Markov Decision Processes}
A Controlled Markov Process (CMP) is a tuple $\mathcal{M} := (\sspace, \aspace, P, D)$, where $\sspace$ is the state space, $\aspace$ is the action space, the transition model $P(s' | a, s)$ denotes the conditional probability of reaching state $s' \in \sspace$ when selecting action $a \in \aspace$ in state $s \in \sspace$, and $D$ is the initial state distribution.
The behavior of an agent is described by a policy $\pi (a | s)$, which defines the probability of taking acion $a \in \aspace$ in $s \in \sspace$. Let $\Pi$ be the set of all the stationary policies.
Executing a policy $\pi \in \Pi$ in a CMP over $T$ steps generates a trajectory $\tau = (s_{0,\tau}, a_{0,\tau}, \ldots, a_{T-2,\tau}, s_{T - 1, \tau})$ with probability
$$
    p_{\pi, \cmp} (\tau) = D(s_{0, \tau}) \prod^{T - 1}_{t = 0} \pi(a_{t,\tau} | s_{t,\tau}) P (s_{t+1,\tau}| s_{t,\tau}, a_{t,\tau}).
$$
We denote the state-visitation frequencies induced by $\tau$ with $ d_\tau (s) = \frac{1}{T} \sum_{t=0}^{T-1} \ind (s_{t,\tau} = s)$, and we call $d_\pi^{\cmp} = \EV_{\tau \sim p_{\pi, \cmp}} [d_{\tau}]$ the marginal state distribution. We define the differential entropy~\citep{shannon1948entropy} of $d_\tau$ as 
$$ 
	H (d_\tau) = - \int_\sspace d_\tau (s) \log d_{\tau} (s) \de s.
$$
For simplicity, we will write $H (d_\tau)$ as a random variable $H_\tau \sim \delta (h - H(d_\tau)) p_{\pi, \cmp} (\tau)$, where $\delta(h)$ is a Dirac delta.

By coupling a CMP $\cmp$ with a reward function $R$ we obtain a Markov Decision Process~\citep[MDP,][]{puterman2014markov} $\cmp^R := \cmp \cup R$. Let $R(s, a)$ be the expected immediate reward when taking $a \in \aspace$ in $s \in \sspace$ and let $R(\tau) = \sum_{t=0}^{T -1} R (s_{t, \tau})$, the \emph{performance} of a policy $\pi$ over the MDP $\cmp^R$ is defined as
\begin{equation}
    \mathcal{J}_{\cmp^R} (\pi) = \EV_{\tau \sim p_{\pi,\cmp}} \big[ R (\tau) \big].
    \label{eq:rl_objective}
\end{equation}
The goal of reinforcement learning~\cite{sutton2018reinforcement} is to find an optimal policy $\pi^*_{\mathcal{J}} \in \arg \max \mathcal{J}_{\cmp^R} (\pi)$ through sampled interactions with an unknown MDP $\cmp^R$.


==> submission/contents/sections/problem.tex <==
\input{contents/figures/problem}
%In this section, we present the objective for \emph{learning to explore multiple environments} with a unique general strategy.
Let $\vcmp = \{\cmp_1, \ldots, \cmp_{I}\}$ be a class of unknown CMPs, in which every  element $\cmp_i = (\sspace, \aspace, P_i, D)$ has a specific transition model $P_i$, while $\sspace, \aspace, D$ are homogeneous across the class. At each turn, the agent is able to interact with a single environment $\cmp \in \vcmp$. The selection of the environment to interact with is mediated by a distribution $p_{\vcmp}$ over $\vcmp$, outside the control of the agent. The aim of the agent is to learn an exploration strategy that is general across all the MDPs $\cmp^R$ one can build upon $\vcmp$. In a single-environment setting, this problem has been assimilated to learning a policy that maximizes the entropy of the induced state visitation frequencies~\citep{hazan2019maxent,lee2019smm,mutti2020policy}. One can straightforwardly extend the objective to multiple environments by considering the expectation over the class of CMPs,
$
    \mathcal{E}_{\vcmp} (\pi) = \EV_{\substack{\cmp \sim p_{\vcmp} \\ \tau \sim p_{\pi, \cmp}}} \big[ H_{\tau} \big],
    %\label{eq:exp_risk_neutral}
$
where the usual entropy objective over the single environment $\cmp_i$ can be easily recovered by setting $p_{\cmp_i} = 1$.
However, this objective function does not account for the tail behavior of $H_\tau$, \ie for the exploration performance in environments of $\vcmp$ that are rare or particularly unfavorable. This is decidedly undesirable as the agent may be tasked with an MDP built upon one of these adverse environments in the subsequent RL phase, where even an optimal strategy \wrt $\mathcal{E}_{\vcmp} (\pi)$ may fail to provide sufficient exploration. To overcome this limitation, we look for a more nuanced exploration objective that balances the expected performance with the sensitivity to the tail behavior. By taking inspiration from the risk-averse optimization literature~\citep{rockafellar2000optimization}, we consider the CVaR of the state visitation entropy induced by $\pi$ over $\vcmp$,
\begin{align}
    \mathcal{E}_{\vcmp}^\alpha (\pi) &= \cvar (H_\tau) \nonumber \\
    &= \EV_{\substack{\cmp \sim p_{\vcmp} \\ \tau \sim p_{\pi, \cmp}}} \big[ H_{\tau} \;|\; H_{\tau} \leq \var (H_\tau) \big],
    \label{eq:exp_risk_averse}    
\end{align}
where $\alpha$ is a confidence level and $\mathcal{E}_{\vcmp}^1 (\pi) := \mathcal{E}_{\vcmp} (\pi)$. The lower we set the value of $\alpha$, the more we hedge against the possibility of a bad exploration outcome in some $\cmp \in \vcmp$.
In the following sections, we propose a method to effectively learn a policy $\pi^*_{\mathcal{E}} \in \arg \max \mathcal{E}_{\vcmp}^\alpha (\pi)$ through mere interactions with $\vcmp$, and we show how this serves as a pre-training for RL (the full process is depicted in Figure~\ref{fig:problem}).

==> submission/contents/sections/related_work.tex <==
Our work lies at the intersection of reward-free exploration, robust and risk-averse RL, and meta-RL. 
%(Figure~\ref{fig:related_work}).
%\begin{wrapfigure}{R}{0.50\textwidth}
%\vspace{-0.5cm}
%\begin{minipage}{0.49\textwidth}
%\input{contents/figures/related_work}
%\end{minipage}
%\end{wrapfigure}

% Entropy Maximization
The literature that relates the most with our work is the one pursuing a \emph{MSVE objective} in reward-free settings. Some methods~\citep{hazan2019maxent,lee2019smm} focus on learning a mixture of policies that is collectively MSVE optimal, while other~\citep{tarbouriech2019active, mutti2020intrinsically} casts the MSVE as a dual (or surrogate) linear program in tabular settings. Successive works tackle MSVE at scale with non-parametric entropy estimation~\citep{mutti2020policy,anonymous2021unsupervised, liu2021aps, yarats2021reinforcement, seo2021state}, or introduce variations to the entropy objective, such as geometry-awareness~\citep{guo2021geometric} and R\'enyi generalization~\citep{zhang2020exploration}. To the best of our knowledge, all existing solutions are environment-specific and do not directly address multiple environments.

% Robust RL and risk-aversion
Previous work considered \emph{CVaR optimization} in RL, either to learn a policy that is averse to the risk induced by the volatility of returns~\citep{tamar2015optimizing,chow2014algorithms} or by changes in the environment dynamics~\citep[\eg][]{rajeswaran2016epopt}. Here we account for a different source of risk, which is the one of running into a particularly unfavorable environment for the trained exploration strategy.

% Meta RL
Finally, the two-stage learning setting we address has clear connections with the \emph{meta-RL} problem setting \citep{finn2017model}, in which we would call meta-training the reward-free phase, and meta-testing the subsequent RL tasks. While some methods target exploration in meta-RL \citep[\eg][]{xu2018meta, gupta2018maesn, zintgraf2019varibad}, they usually assume access to rewards during meta-training, with the notable exception of~\citep{gupta2018unsupervised}. To the best of our knowledge, none of the existing works combine reward-free meta-training with a multiple-environments setting.

==> submission/contents/sections/theory.tex <==
We aim to theoretically analyze the problem in~\eqref{eq:exp_risk_averse}, and especially, what makes a class of multiple CMPs hard to explore with a unique strategy. This has to be intended as a preliminary discussion on the problem, which could serve as a starting point for future works, rather than a thorough theoretical characterization.
First, it is worth introducing some additional notation.

\paragraph{Lipschitz Continuity}
Let $X,Y$ be two metric sets with metric functions $d_X, d_Y$. We say a function $f:X \to Y$ is $L_f$-Lipschitz continuous if it holds for some constant $L_f$
$$
    d_Y (f(x'), f(x)) \leq L_f d_X (x',x), \forall (x',x) \in X^2,
$$
where the smallest $L_f$ is the Lipschitz constant and the Lipschitz semi-norm is $\norm{f}{L} = \sup_{x',x \in X} \big\lbrace \frac{d_Y (f(x'), f(x))}{d_X (x',x)} : x' \neq x \big\rbrace$.
When dealing with probability distributions we need to introduce a proper metric. Let $p,q$ be two probability measures, we will either consider the Wasserstein metric~\citep{villani2008optimal}, defined as
$$
    \wass (p, q) = \sup_{f} \big\lbrace \big| \int_X f (x) (p(x) - q(x)) \de x \big| : \norm{f}{L} \leq 1 \big\rbrace,
$$
or the Total Variation (TV) metric, defined as
$$
    d_{TV} (p, q) = \frac{1}{2} \int_X \big| p(x) - q(x)  \big| \de x.
$$

Intuitively, learning to explore a class $\vcmp$ with a policy $\pi$ is challenging when the state distributions induced by $\pi$ in different $\cmp \in \vcmp$ are diverse. The more diverse they are, the more their entropy can vary, and the harder is to get a $\pi$ with a large entropy across the class. To measure this diversity, we are interested in the supremum over the distances between the state distributions $(d_{\pi}^{\cmp_1}, \ldots, d_{\pi}^{\cmp_I})$ that a single policy $\pi \in \Pi$ realizes over the class $\vcmp$. We call this measure the \emph{diameter} $\diam_{\vcmp}$ of the class $\vcmp$. Since we have infinitely many policies in $\Pi$, computing $\diam_{\vcmp}$ is particularly arduous. However, we are able to provide an upper bound to $\diam_{\vcmp}$ defined through a Wasserstein metric.
\begin{restatable}[]{ass}{lipschitz_assumption}
    Let $d_{\sspace}$ be a metric on $\sspace$. The class $\vcmp$ is $L_{P^\pi}$-Lipschitz continuous,
    \begin{equation*}
        \wass( P^\pi (\cdot| s'), P^\pi (\cdot| s)) \leq L_{P^\pi} d_{\sspace} (s',s),
        \;\; \forall (s',s) \in \sspace^2,
    \end{equation*}
    where $P^\pi (s|\os) = \int_{\aspace} \pi (\oa|\os) P(s | \os, \oa) \de \oa$ for $P \in \vcmp$, $\pi \in \Pi$, $L_{P^\pi}$ is a constant $L_{P^\pi} < 1$.
    \label{ass:lipschitz}
\end{restatable}
\begin{restatable}[]{thm}{diameter}
    Let $\vcmp$ be a class of CMPs satisfying Ass.~\ref{ass:lipschitz}. Let $d^{\cmp}_{\pi}$ be the marginal state distribution over $T$ steps induced by the policy $\pi$ in $\cmp \in \vcmp$. We can upper bound the diameter $\diam_{\vcmp}$  as
    \begin{align}
        \diam_{\vcmp} := \sup_{\pi \in \Pi,\; \cmp', \cmp \in \vcmp} 
        \wass (d_{\pi}^{\cmp'}, d_{\pi}^{\cmp}) \leq \sup_{P',P \in \vcmp} \frac{1 - L_{P^\pi}^T}{1 - L_{P^\pi}}
        \sup_{s \in \mathcal{S},a \in \mathcal{A}} 
        \wass (P'(\cdot|s,a), P (\cdot|s,a)). \nonumber
    \end{align}
    \label{thm:dimater}
\end{restatable}
Theorem~\ref{thm:dimater} provides a measure to quantify the hardness of the exploration problem in a specific class of CMPs, and to possibly compare one class with another. However, the value of $\diam_{\vcmp}$ might result, due to the supremum over $\Pi$, from a policy that is far away from the policies we actually deploy while learning, say $(\pi_0, \ldots, \pi_{\mathcal{E}}^*)$. To get a finer assessment of the hardness of $\vcmp$ we face in practice, it is worth considering a policy-specific measure to track during the optimization. We call this measure the \emph{$\pi$-diameter} $\diam_{\vcmp} (\pi)$ of the class $\vcmp$. Theorem~\ref{thm:pi_dimater} provides an upper bound to $\diam_{\vcmp} (\pi)$ defined through a convenient TV metric.
\begin{restatable}[]{thm}{piDiameter}
    Let $\vcmp$ be a class of CMPs, let $\pi \in \Pi$ be a policy, and let $d^{\cmp}_{\pi}$ be the marginal state distribution over $T$ steps induced by $\pi$ in $\cmp \in \vcmp$. We can upper bound the $\pi$-diameter $\diam_{\vcmp} (\pi)$ as
    \begin{align}
        \diam_{\vcmp} (\pi) := \sup_{\cmp', \cmp \in \vcmp} 
        d_{TV} (d_{\pi}^{\cmp'}, d_{\pi}^{\cmp}) \leq \sup_{P',P \in \vcmp} T \EV_{\substack{s \sim d_{\pi}^{\cmp} \\ a \sim \pi(\cdot|s)}}
        d_{TV} (P'(\cdot|s,a), P (\cdot|s,a)). \nonumber
    \end{align}
    \label{thm:pi_dimater}
\end{restatable}
The last missing piece we aim to derive is a result to relate the $\pi$-diameter $\diam_{\vcmp} (\pi)$ of the class $\vcmp$ (Theorem~\ref{thm:pi_dimater}) with the actual exploration objective, \ie the entropy of the state visitations induced by the policy $\pi$ over the environments in the class. In the following theorem, we provide an upper bound to the \emph{entropy gap} induced by the policy $\pi$ within the class $\vcmp$.
\begin{restatable}[]{thm}{entropyDiameter}
    Let $\vcmp$ be a class of CMPs, let $\pi \in \Pi$ be a policy and $\diam_{\vcmp} (\pi)$ the corresponding $\pi$-diameter of $\vcmp$. Let $d^{\cmp}_{\pi}$ be the marginal state distribution over $T$ steps induced by $\pi$ in $\cmp \in \vcmp$, and let $\sigma_{\vcmp} \leq \sigma_{\cmp} := \inf_{s \in \sspace} d^{\cmp}_{\pi} (s), \forall \cmp \in \vcmp$. We can upper bound the entropy gap of the policy $\pi$ within the model class $\vcmp$ as
    \begin{align}
        \sup_{\cmp',\cmp \in \vcmp} \big|  H (d_{\pi}^{\cmp'}) - H (d_{\pi}^{\cmp}) \big| \leq \big( \diam_{\vcmp} (\pi) \big)^2 \big/ \sigma_{\vcmp} + \diam_{\vcmp} (\pi) \log  (1  / \sigma_{\vcmp}) \nonumber
    \end{align}
    \label{thm:entropy_dimater}
\end{restatable}

